Fibered Correspondence

Base of fibered correspondence is arbitrary correspondence. Fibered correspondence is interesting when we consider relationship between different bundles. However composition of fibered correspondences may not always be defined. Reduced fibered correspondence is defined only between fibers over the same point of base. Reduced fibered correspondence in bundle is called 2-ary fibered relation. We considered fibered equivalence and isomorphism theorem in case of fibered morphisms.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{texIntro}{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84 (1966)
}%

\BiblioItem{texGenRelativity}{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{texGenRelativity}{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{texAffine}{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{texAffine}{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric-affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{texAffine}{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{texAffine}{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\BiblioItem{texAffine}{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%

\BiblioItem{texAffine}{0405.027}
{
Aleks Kleyn,
Reference Frame in General Relativity,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2004)
}%

\BiblioItem{texTidal,texAffine}{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{texTidal,texNewton}{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{texNewton}{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{texNewton}{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric-affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{texLagrange}{Weinberg}
{
Steven Weinberg. The Quantum Theory of Fields. Cambridge university press.
}%

\BiblioItem{texLagrange}{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{texLagrange}{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{texTidal}{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{texTidal}{0405.028}
{
Aleks Kleyn, Metric-Affine Manifold,
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2004)
}%

\BiblioItem{texTidal}{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{texTidal}{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{texReferenceFrame,texFiberedAlgebra}{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{texFiberedAlgebra,texTstarMorphism}{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

%\BiblioItem{texBasis}{Shilov}
%{
%Г. Е. Шилов, Математический анализ,
%Функции нескольких вещественных переменных, части 1 - 2,
%М., Наука, 1972
%}%

\BiblioItem{texAffine,texRepresentation,texBasis,texDrcBasis,texVectorSpace,texLinearMap}
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem{texDrcBasis,texBasis}{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{texGenRelativity}{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{texGenRelativity}{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{texGenRelativity}{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{texGenRelativity}{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{texGenRelativity}{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity}{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity}{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity,texTidal}{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{texBiring,texVectorSpace}{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{texBiring,texVectorSpace}
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{texVectorSpace}{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{texVectorSpace}{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{texVectorSpace}{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{texVectorSpace}{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{texReferenceFrame}{math.DG-0412391}
{
Александр Клейн,
Frame Manifold,
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2004)
}%

\BiblioItem{texFiberedAlgebra,texBundleRelation,texTstarMorphism}{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2007)
}%

\BiblioItem{texBundleRelation,texPrefaceRelation}{0702.561}
{
Александр Клейн,
Расслоенная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

%\BiblioItem{texBasis,texLinearMap}{math.RA-0501237}
%{
%Александр Клейн,
%Векторное пространство над телом,\\
%eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2005)
%}%

\BiblioItem{texPolymodule}{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Skew-Field, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\ifx\texBiring\Defined
\else
\BiblioItem{texVectorSpace,texFiberedAlgebra}{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2006)
}%
\fi

\ifx\texBundleRelation\Defined
\else
\BiblioItem{texFiberedMorphism}{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%
\fi

\BiblioItem{texHomotopy}{q-alg-9705009}
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{texIntro}{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81 (1967)
}%

\BiblioItem{texPrefaceRelation}{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem{texBundleRelation,texPrefaceRelation,texTstarMorphism,texCartesian}
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem{texCartesian}
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{texFiberedAlgebra}{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{texBundleRelation}{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{texCartesian,texFiberedAlgebra,texBundleRelation,texFiberedMorphism}
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{texCalculus}{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{texCalculus}{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{texCalculus}{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem{texFiberedMorphism}{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{texFiberedAlgebra,texFiberedMorphism}{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{texFiberedMorphism}{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{texFiberedMorphism}{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\CloseBiblio



==> Fibered.Morphism.Russian.tex <==
%auto-ignore
\def\texFiberedMorphism{}
\ifx\PrintBook\Defined
				\chapter{Расслоенный морфизм}
\fi

			\section{Расслоенный морфизм}

		\begin{theorem}
		\label{theorem: quotient bundle}
Пусть на расслоении $\bundle{\mathcal{E}}pEM$
определена расслоенная эквивалентность $\bundle{\mathcal{S}}sSM$.
Тогда существует расслоение
\[\bundle{\mathcal{E}/\mathcal{S}}t{E/S}M\]
называемое \AddIndex{фактор расслоением}{quotient bundle}
расслоения $\mathcal{E}$ по
эквивалентности $\mathcal{S}$.
Морфизм расслоений
\[
\mathrm{nat}\mathcal{S}:\mathcal{E}\rightarrow
\mathcal{E}/\mathcal{S}
\]
называется \AddIndex{расслоенным естественным морфизмом}{fibered natural morphism}
или \AddIndex{расслоенным морфизмом отождествления}{fibered identification morphism}.
		\end{theorem}
		\begin{proof}
Рассмотрим коммутативную диаграмму
\begin{equation}
\label{eq: quotient bundle}
\xymatrix{
\mathcal{E}\ar[rr]^{\mathrm{nat}\mathcal{S}}\arp[rd]_{\bundle{}pE{}}
&&\mathcal{E}/\mathcal{S}\arp[dl]^{\bundle{}t{E/S}{}}\\
&M&
}
\end{equation}
Мы определим в $\mathcal{E}/\mathcal{S}$ фактортопологию
(\citeBib{Bourbaki: General Topology 1}, стр. 39),
требуя непрерывность отображения $\mathrm{nat}\mathcal{S}$.
Согласно предложению \citeBib{Bourbaki: General Topology 1}-I.3.6
отображение $\bundle{}t{E/S}{}$ непрерывно.

Так как эквивалентность $S$ определена только между точками
одного слоя $E$, то классы эквивалентности принадлежат
одному и тому слою $E/S$ (сравни с замечанием к предложению
\citeBib{Bourbaki: General Topology 1}-I.3.6).
		\end{proof}

Пусть $f:\mathcal{A}\rightarrow\mathcal{B}$ -
расслоенный морфизм, база которого является
тождественным отображением.
Согласно определению
\xRef{0707.2246}{definition: inverse reduced fibered correspondence}
существует обратное приведенное расслоенное соответствие $f^{-1}$.
Согласно теоремам
\xRef{0707.2246}{theorem: composition of reduced fibered correspondences}
и \xRef{0707.2246}{theorem: 2 ary fibered relation}
$f^{-1}\circ f$ является $2$\Hyph арным расслоенным отношением.

		\begin{theorem}
Расслоенное отношение $\mathcal{S}=f^{-1}\circ f$ является
расслоенной эквивалентностью на расслоении $\mathcal{A}$.
Существует разложение расслоенного морфизма $f$ в произведение
расслоенных морфизмов
	\begin{equation}
f=itj
	\label{eq: morphism of representations of algebra, homomorphism, 1}
	\end{equation}
\[
\xymatrix{
\mathcal{A}/\mathcal{S}\ar[rr]^t&&f(\mathcal{A})\ar[d]^i\\
\mathcal{A}\ar[u]^j\ar[rr]^f&&\mathcal{B}
}
\]
$j=\mathrm{nat}\mathcal{S}$ - естественный гомоморфизм
	\begin{equation}
\textcolor{red}{j(a)}=j(a)
	\label{eq: morphism of representations of algebra, homomorphism, 2}
	\end{equation}
$t$ - изоморфизм
	\begin{equation}
\textcolor{red}{r(a)}=t(\textcolor{red}{j(a)})
	\label{eq: morphism of representations of algebra, homomorphism, 3}
	\end{equation}
$i$ - вложение
	\begin{equation}
r(a)=i(\textcolor{red}{r(a)})
	\label{eq: morphism of representations of algebra, homomorphism, 4}
	\end{equation}
		\end{theorem}
		\begin{proof}
Утверждение теоремы проверяется в слое. Необходимо
также проверить, что эквивалентность непрерывно зависит от слоя.

%Пусть $x\in M$, $p\in A$, $q\in A$,
%$(x,p)\in A_x$, $(x,q)\in A_x$. Положим $R_x=f_x^{-1}\circ f_x$.
%Положим, $(p,q)\in R_x$.
%Пусть $U\subset M$ - открытое множество, $x\in U$.
%Положим $r=f_x(p)\in B$.
%Пусть $U_B\subset B$ - открытое множество, $r\in U_B$.
%Поскольку $f$ - непрерывное отображение, то существуют
%открытые множества $U_p\subset A$, $p\in U_p$, $f(U_p)\subset U_B$,
%$U_q\subset A$, $p\in U_q$, $f(U_q)\subset U_B$.
		\end{proof}

\section{Свободное \texorpdfstring{$T\star$}{T*}-представление
расслоенной группы}

Отображение $\mathrm{nat}\mathcal{S}$ не порождает расслоения,
так как разные классы эквивалентности, вообще говоря, не гомеоморфны.
Однако доказательство теоремы \ref{theorem: quotient bundle}
подсказывает конструкцию, очень напоминающую построение,
предложенное в \citeBib{Postnikov: Differential Geometry}, стр. 16 - 17.

	 \begin{definition}
	 \label{definition: fibered little group}
Рассмотрим \Ts представление $f$ расслоенной группы $\bundle{}pG{}$
в расслоении $\mathcal{M}$.
\AddIndex{Расслоенная малая группа}{fibered little group} или
\AddIndex{расслоенная группа стабилизации}{fibered stability group}
сечения $h\in \Gamma(\mathcal{M})$ -
это множество
\symb{\mathcal{G}_h}0{fibered little group}
\symb{\mathcal{G}_h}0{fibered stability group}
\[
\ShowSymbol{fibered little group}=\{g\in \Gamma(\mathcal{G}):f(g)h=h\}
\]
	 \qed
	 \end{definition}

		\begin{theorem}
		\label{theorem: fibered little group}
Рассмотрим \Ts представление $f$ расслоенной группы $\bundle{}pG{}$
в расслоении $\bundle{\mathcal{E}}rEM$.
Допустим $\mathcal{G}_h$ - расслоенная малая группа
сечения $h$. Для любого $x\in M$ слой $\mathcal{G}_{h,x}$
расслоенной малой группы
сечения $h$ является подгруппой малой группы
$G_{h(x)}$ элемента $h(x)\in E_x$.
		\end{theorem}
		\begin{proof}
Выберем сечение $g\in\Gamma(\mathcal{G}_h)$ так,
что преобразование $f(g)$ оставляет неподвижным
сечение $h\in\Gamma(\mathcal{E})$. Следовательно, преобразование
$f(h(x))$ оставляет неподвижным $h(x)\in E_x$.
		\end{proof}

	 \begin{definition}
	 \label{definition: free representation of fibered group}
Мы будем называть \Ts представление $f$ расслоенной группы $\bundle{}pG{}$
\AddIndex{свободным}{free representation of fibered group},
если для любого $x\in M$ \Ts представление $f_x$
группы $G_x$ в слое $E_x$ свободно.
	 \qed
	 \end{definition}

		\begin{theorem}	%
		\label{theorem: free representation of group}
Если определено свободное \Ts представление $f$ расслоенной группы
$\bundle{}pG{}$ в расслоении $\bundle{\mathcal{E}}rEM$,
то определено взаимно однозначное соответствие
между орбитой представления в слое и группой $G$.
Если группа $G$ - топологическая группа, то орбита представления в слое
гомеоморфна группе $G$.
		\end{theorem}
		\begin{proof}
		\end{proof}

Рассмотрим ковариантное свободное \Ts представление $f$
расслоенной группы $\bundle{}pG{}$ на расслоении $\bundle{}pE{}$.
Это \Ts представление определяет на $\bundle{}aE{}$ расслоенное отношение
эквивалентности $\mathcal{S}$, $(p,q)\in S$ если $p$ и $q$ принадлежат
общей орбите. 
Так как представление в каждом слое свободно,
все классы эквивалентности гомеоморфны группе $G$.
Следовательно, отображение $\mathrm{nat}\mathcal{S}$
является проекцией расслоения
$\bundle{\mathcal{E}}{\mathrm{nat}\mathcal{S}}G{\mathcal{E}/\mathcal{S}}$.
Мы также будем пользоваться символом $\mathcal{S}=\mathcal{G}\star$.
Мы можем представить диаграмму \eqref{eq: quotient bundle}
в виде конструкции
\[
\xymatrix{
\mathcal{E}\arp[drr]^{\bundle{}{\mathrm{nat}\mathcal{S}}G{}}
\arp[dd]^{\bundle{}pE{}}&&\\
&&\mathcal{E}/\mathcal{S}\arp[dll]^{\bundle{}t{E/S}{}}\\
M&&
}
\]
Мы будем называть расслоение $\bundle{}{\mathrm{nat}\mathcal{S}}G{}$
\AddIndex{расслоением уровня $2$}{bundle of level 2}.

\begin{example}
Рассмотрим представление группы вращений $SO(2)$ в $R^2$.
Все точки, кроме точки
$(0,0)$, имеют тривиальную малую группу.
Таким образом, на множестве $R^2\setminus \{(0,0)\}$
определено свободное представление группы $SO(2)$.

Мы не можем воспользоваться этой операцией в случае расслоения
$\bundle{}p{R^2}{}$ и представления расслоенной группы $\bundle{}t{SO(2)}{}$.
Пусть $\mathcal{S}$ - отношение расслоенной эквивалентности.
Расслоение $\bundle{}p{R^2\setminus \{(0,0)\}}{}/\bundle{}t{SO(2)}{}\star$
не является полным. В результате предельный переход может привести в
несуществующий слой. Поэтому мы предпочитаем рассматривать
расслоение $\bundle{}p{R^2}{}/\bundle{}t{SO(2)}{}\star$,
имея в виду, что слой над точкой $(x,0,0)$ - вырожден.
	 \qed
\end{example}

Мы упростим обозначения и представим полученную конструкцию в виде
\symb{p[E_2,E_1]}0{bundle of level 2}
\[
\xymatrix{
\ShowSymbol{bundle of level 2}:\mathcal{E}_2\arp[r]&
\mathcal{E}_1\arp[r]&
M
}
\]
где мы предполагаем расслоения
\begin{align*}
\bundle{\mathcal{E}_2}{p_2}{E_2}{\mathcal{E}_1}&&
\bundle{\mathcal{E}_1}{p_1}{E_1}M&
\end{align*}
Аналогичным образом мы можем рассматривать
\AddIndex{расслоение уровня $n$}{bundle of level n}
\symb{p[E_n,...,E_1]}0{bundle of level n}
\begin{equation}
\label{eq: bundle of level n}
\xymatrix{
\ShowSymbol{bundle of level n}:\mathcal{E}_n\arp[r]&\ar@{}[r]_{...}&\arp[r]&
\mathcal{E}_1\arp[r]&
M
}
\end{equation}
Последовательность расслоений \eqref{eq: bundle of level n}
мы будем называть \AddIndex{башней расслоений}{tower of bundles}.
Это определение я дал по аналогии с башней Постникова
(\citeBib{Hatcher: Algebraic Topology}).
Башня Постникова - это башня расслоений. Слой расслоения уровня $n$ - это
гомотопическая группа порядка $n$.
Подобные конструкции известны, однако я привёл определение башни
расслоений, поскольку оно естественным образом возникает из
вышеизложенного текста.

Я хочу рассмотреть ещё один пример башни расслоений, который
привлёк моё внимание (\citeBib{geometry of differential equations},
\citeBib{cohomological analysis}, часть 2).
В качестве базы выберем множество $J^0(n,m)$ $0$\Hyph джетов
отображений из $R^n$ в $R^m$. В качестве расслоения уровня $p$
выберем множество $J^p(n,m)$ $p$\Hyph джетов
отображений из $R^n$ в $R^m$.


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index{texLinearMap}%1%1
   {$1$-\drc форма}%
   {1-drc form, vector spaces}%
\SetIndexSpace%
\Index{texPolymodule}%2%66
   {$(2)$\hyph векторное пространство}%
   {(2)-vector space}%
\Index{texBundleRelation}%2%122
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index{texBiring}%A%2
   {$(^{\gi a}_{\gi b})$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index{texBiring}%A%34
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant}%
\Index{texCalculus}%A%67
   {$A$\Hyph значная функция}%
   {A valued function}%
\SetIndexSpace%
\Index{texBiring}%C%3
   {\subs строка матрицы}%
   {c row}%
\Index{texVectorSpace}%C%5
   {\CR матричная группа}%
   {cr-matrix group}%
\Index{texBiring}%C%6
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index{texBiring}%C%7
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index{texBiring}%C%8
   {\CR степень}%
   {cr power}%
\Index{texVectorSpace}%C%9
   {\crd векторное пространство}%
   {crd vector space}%
\Index{texBiring}%C%10
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index{texVectorSpace}%D%11
   {\dcr базис векторного пространства \subs строк}%
   {dcr basis, c rows vector space}%
\Index{texVectorSpace}%D%12
   {\dcr вектор}%
   {dcr vector}%
\Index{texVectorSpace}%D%13
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index{texVectorSpace}%D%14
   {\dcr векторное пространство \subs строк}%
   {subs rows dcr vector space}%
\Index{texVectorSpace}%D%15
   {\drc  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index{texVectorSpace}%D%55
   {\drc автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index{texVectorSpace}%D%17
   {\drc базис}%
   {}%
\SubIndex{texVectorSpace}%4%
   {в векторном пространстве}%
   {drc basis, vector space}%
\SubIndex{texVectorSpace}%5%
   {в векторном пространстве \sups строк}%
   {drc basis, r rows vector space}%
\Index{texVectorSpace}%D%18
   {\drc вектор}%
   {drc vector}%
\Index{texVectorSpace}%D%19
   {\drc векторное пространство}%
   {drc vector space}%
\Index{texVectorSpace}%D%20
   {\drc векторное пространство \sups строк}%
   {sups rows drc vector space}%
\Index{texCalculus}%D%46
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index{texVectorSpace}%D%83
   {\drc изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index{texVectorSpace}%D%87
   {\drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Index{texVectorSpace}%D%23
   {\drc линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index{texReferenceFrame}%D%24
   {\drc линейно независимыe векторы}%
   {linearly independent vector fields}%
\Index{texVectorSpace}%D%114
   {\drc линейно независимые векторы}%
   {linearly independent, vector space}%
\Index{texDrcMorphism}%D%25
   {\drc линейное отображение векторных пространств}%
   {drc linear map of vector spaces}%
\Index{texVectorSpace}%D%27
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index{texVectorSpace}%D%26
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index{texCalculus}%D%96
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\SetIndexSpace%
\Index{texELie}%E%28
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index{texDiffEq}%E%29
   {essential parameters}%
   {essential parameters}%
\SetIndexSpace%
\Index{texTypeBasis}%G%30
   {\Gbasis}%
   {G-basis}%
\Index{texTypeBasis}%G%31
   {\Gcoords ы}%
   {G-coordinates}%
\Index{texTypeBasis}%G%32
   {\Gspace о}%
   {GSpace}%
\Index{texBasis}%G%267
   {\Gbasis\ векторного пространства}%
   {G-basis}%
\Index{texBasis}%G%270
   {\Gcoords ы базиса}%
   {G-coordinates}%
\Index{texBasis}%G%271
   {\Gspace о}%
   {GSpace}%
\SetIndexSpace%
\Index{texPolymodule}%N%231
   {$(n)$\hyph векторное пространство}%
   {(n)-vector space}%
\Index{texBundleRelation}%N%218
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index{texBiring}%R%35
   {\sups строка матрицы}%
   {r row}%
\Index{texVectorSpace}%R%36
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index{texVectorSpace}%R%37
   {\RC главный минор}%
   {RC-major minor}%
\Index{texBiring}%R%38
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index{texVectorSpace}%R%39
   {\RC матричная группа}%
   {rc-matrix group}%
\Index{texVectorSpace}%R%40
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index{texBiring}%R%41
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index{texBiring}%R%42
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index{texVectorSpace}%R%43
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index{texBiring}%R%44
   {\RC степень}%
   {rc power}%
\Index{texVectorSpace}%R%45
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index{texVectorSpace}%R%213
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index{texBiring}%R%47
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index{texDrcMorphism}%S%314
   {$(S\RCstar,T\RCstar)$\Hyph линейное отображение векторных пространств}%
   {src trc linear map of vector spaces}%
\Index{texLinearMap}%S%48
   {$\star D$\Hyph произведением \drc линейного отображения $A$ на скаляр}%
   {starD product of drc linear map over scalar}%
\Index{texVectorSpace}%S%217
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index{texVectorSpace}%S%216
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index{texTstarRepresentation}%S%49
   {\sT сдвиг}%
   {starT shift}%
\Index{texFiberedGroup}%S%50
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\Index{texTstarMorphism}%S%160
   {\sT представление $\mathcal{F}$\Hyph алгебры $A$ в множестве $M$}%
   {starT representation of algebra}%
\Index{texFiberedAlgebra}%S%162
   {\sT представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {starT representation of fibered F-algebra}%
\Index{texFiberedGroup}%S%163
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index{texTstarMorphism}%S%308
   {\sT преобразование}%
   {starT transformation}%
\Index{texFiberedAlgebra}%S%167
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\SubIndex{}%71%
   {невырожденное}%
   {nonsingular transformation of bundle}%
\SetIndexSpace%
\Index{texVectorSpace}%T%51
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index{texVectorSpace}%T%52
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index{texFiberedGroup}%T%316
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\Index{texTstarRepresentation}%T%53
   {\Ts сдвиг}%
   {Tstar shift}%
\Index{texTstarMorphism}%T%301
   {\Ts представление $\mathcal{F}$\Hyph алгебры $A$ в множестве $M$}%
   {Tstar representation of algebra}%
\Index{texFiberedAlgebra}%T%321
   {\Ts представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {Tstar representation of fibered F-algebra}%
\Index{texTstarMorphism}%T%309
   {\Ts преобразование}%
   {Tstar transformation}%
\Index{texFiberedAlgebra}%T%327
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\SetIndexSpace%
\Index{texNewton}%V%54
   {vector potential}%
   {vector potential}%
\SetIndexSpace%
\Index{texAffine}%А%56
   {автопараллельная кривая}%
   {auto parallel line}%
\Index{texDrcBasis}%А%57
   {активное \sT представление}%
   {active representation, vector space}%
\Index{texBasis}%А%262
   {активное представление}%
   {active representation}%
\Index{texBasis}%А%263
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index{texLie}%А%58
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\SubIndex{texLie}%9%
   {определённая слева}%
   {left defined algebra Lie}%
\SubIndex{texLie}%10%
   {определённая справа}%
   {right defined algebra Lie}%
\Index{texBiring}%А%59
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index{texFiberedGroup}%А%60
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index{texBundleRelation}%А%156
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index{texFiberedAlgebra}%А%61
   {арность операции}%
   {arity of operation}%
\Index{texBasis}%А%277
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index{texBasis}%А%275
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index{texCartesian}%Б%172
   {база отображения}%
   {base of map}%
\Index{texBundleRelation}%Б%233
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index{texTypeBasis}%Б%16
   {базис}%
   {}%
\SubIndex{texTypeBasis}%1%
   {аффинный}%
   {Affine Basis}%
\SubIndex{texTypeBasis}%2%
   {ортонормальный}%
   {Orthonornal Basis}%
\SubIndex{texTypeBasis}%3%
   {центро-аффинный}%
   {Central Affine Basis}%
\Index{texBasis}%Б%266
   {базис векторного пространства}%
   {Basis}%
\Index{texLieRepresentation}%Б%62
   {базовый вектор}%
   {}%
\SubIndex{texLieRepresentation}%11%
   {\sT представления}%
   {basis vector of starT representation}%
\SubIndex{texLieRepresentation}%12%
   {\Ts представления}%
   {basis vector of Tstar representation}%
\Index{texLie}%Б%63
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index{texFiberedMorphism}%Б%351
   {башня расслоений}%
   {tower of bundles}%
\Index{texLieRepresentation}%Б%64
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index{texBiring}%Б%65
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index{texPolymodule}%В%230
   {($D_1\RCstar$, ..., $D_n\RCstar$)\hyph векторное пространство}%
   {(d1rc,dnrc)-vector space}%
\Index{texPolymodule}%В%229
   {($S\star$, $\star T$)\hyph векторное пространство}%
   {(Sstar,starT)-vector space}%
\Index{texDiffProperty}%В%69
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index{texRepresentation}%В%261
   {вектор\hyph столбец}%
   {column vector}%
\Index{texFiberedAlgebra}%В%70
   {векторное расслоение}%
   {vector bundle}%
\Index{texRepresentation}%В%260
   {вектор\hyph строка}%
   {row vector}%
\Index{texDiffEq}%В%71
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index{texNewton}%В%72
   {второй закон Ньютона}%
   {Second Newton law}%
\SetIndexSpace%
\Index{texDrcBasis}%Г%73
   {геометрический объект}%
   {}%
\SubIndex{texDrcBasis}%13%
   {в координатном представлении,	определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\SubIndex{texDrcBasis}%14%
   {определённый в векторном пространстве}%
   {geometrical object, vector space}%
\SubIndex{texDrcBasis}%15%
   {типа $A$}%
   {geometrical object of type A, vector space}%
\Index{texBasis}%Г%290
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%
\Index{texBasis}%Г%288
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Index{texBasis}%Г%293
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometrical object of type A, vector space}%
\Index{texReferenceFrame}%Г%74
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index{texFiberedAlgebra}%Г%75
   {гомоморфизм расслоенных $\mathcal{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Index{texFiberedGroup}%Г%76
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index{texTypeBasis}%Г%77
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%274
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%264
   {группа симметрии}%
   {symmetry group}%
\Index{texDrcBasis}%Г%78
   {группа симметрии}%
   {SymmetryGroup}%
\Index{texTstarRepresentation}%Г%344
   {группа стабилизации}%
   {stability group}%
\Index{texGroupRing}%Г%79
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index{}%Д%283
   {движение на многообразии базисов}%
   {movement transformation}%
\Index{texCartesian}%Д%331
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index{texCartesian}%Д%176
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Index{texCartesian}%Д%180
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index{texCartesian}%Д%181
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index{texBundleRelation}%Д%113
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index{texBundleRelation}%Д%227
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index{texCalculus}%Д%105
   {дифференциал отображения нормированного \drc векторного пространства в нормированное тело}%
   {differential, drc vector space to skew field}%
\Index{texCalculus}%Д%99
   {дифференцируемая функция \drc векторного пространства в тело $D$ }%
   {differentiable functions, drc vector space to skew field}%
\SetIndexSpace%
\Index{texDrcMorphism}%З%312
   {закон ассоциативности для \drc линейных отображений векторных пространств}%
   {associative law for drc linear maps of vector spaces}%
\Index{texVectorSpace}%З%310
   {закон ассоциативности для \Ts векторного пространства}%
   {associative law, Tstar vector space}%
\Index{texTstarRepresentation}%З%80
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for Tstar covariant representation}%
\Index{texLinearMap}%З%311
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index{texBundleRelation}%З%155
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index{texVectorSpace}%З%81
   {закон дистрибутивности}%
   {}%
\SubIndex{texVectorSpace}%20%
   {\Ts векторное пространство}%
   {distributive law, Tstar vector space}%
\Index{texVectorSpace}%З%82
   {закон унитарности}%
   {}%
\SubIndex{texVectorSpace}%21%
   {для \Ts векторного пространства}%
   {unitarity law, Tstar vector space}%
\SetIndexSpace%
\Index{texFiberedAlgebra}%И%84
   {изоморфизм расслоенных алгебр}%
   {isomorphism of fibered F-algebras}%
\Index{texLinearLie}%И%85
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index{texHomotopy}%К%4
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index{texBundleRelation}%К%111
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index{texBundleRelation}%К%112
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index{texBasis}%К%278
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index{texBasis}%К%284
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index{texFiberedGroup}%К%318
   {ковариантное \Ts представление расслоенной группы}%
   {Tstar covariant representation of fibered group}%
\Index{texBundleRelation}%К%228
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index{texCartesian}%К%332
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index{texFiberedGroup}%К%317
   {контравариантное \Ts представление расслоенной группы}%
   {Tstar contravariant representation of fibered group}%
\Index{texVectorSpace}%К%21
   {координатная матрица}%
   {}%
\SubIndex{texVectorSpace}%6%
   {вектора в \drc базисе}%
   {coordinate matrix of vector in drc basis}%
\SubIndex{texVectorSpace}%7%
   {множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\SubIndex{texVectorSpace}%8%
   {множества векторов в векторном пространстве \drc строк}%
   {coordinate matrix of set of vectors, drc vector space}%
\Index{texReferenceFrame}%К%86
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index{texGenRelativity}%К%239
   {координатная система отсчёта в пространстве событий}%
   {coordinate reference frame in event space}%
\Index{texBasis}%К%285
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index{texDrcBasis}%К%88
   {координатное представление в \drc векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%287
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%286
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%89
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%22
   {координаты вектора в \drc базисе}%
   {coordinates of vector in drc basis}%
\Index{texDrcBasis}%К%90
   {координаты геометрического объекта}%
   {}%
\SubIndex{texDrcBasis}%22%
   {в векторном пространстве}%
   {coordinates of geometrical object, vector space}%
\SubIndex{texDrcBasis}%23%
   {в координатном векторном пространстве}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texBasis}%К%291
   {координаты геометрического объекта}%
   {coordinates of geometrical object, vector space}%
\Index{texBasis}%К%289
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texVectorSpace}%К%91
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index{texVectorSpace}%К%92
   {координаты множества векторов в \drc векторном пространстве}%
   {coordinates of set of vectors, drc vector space}%
\Index{texDrcBasis}%К%93
   {координаты представления}%
   {coordinates of representation}%
\Index{texBasis}%К%265
   {координаты представления}%
   {coordinates of representation}%
\Index{texAffine}%К%94
   {кривизна Картана}%
   {Cartan curvature}%
\Index{texAffine}%К%95
   {кручение}%
   {torsion}%
\SetIndexSpace%
\Index{texVectorSpace}%Л%98
   {левое векторное пространство}%
   {left vector space}%
\Index{texLie}%Л%101
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index{texRepresentation}%Л%247
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation}%
\Index{texRepresentation}%Л%249
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation}%
\Index{texTstarMorphism}%Л%302
   {левостороннее представление $\mathcal{F}$\Hyph алгебры $A$ в множестве $M$}%
   {left-side representation of algebra}%
\Index{texRepresentation}%Л%244
   {левостороннее представление группы}%
   {left-side representation of group}%
\Index{texFiberedAlgebra}%Л%322
   {левостороннее представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {left-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%Л%164
   {левостороннее преобразование}%
   {left-side transformation}%
\Index{texFiberedAlgebra}%Л%328
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index{texLie}%Л%103
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index{texVectorSpace}%Л%214
   {левый модуль}%
   {left module}%
\Index{texTstarRepresentation}%Л%108
   {левый сдвиг}%
   {left shift}%
\Index{texRepresentation}%Л%251
   {левый сдвиг на группе}%
   {left shift, group}%
\Index{texFiberedGroup}%Л%109
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index{texReferenceFrame}%Л%110
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index{texRepresentation}%Л%240
   {линейное представление группы}%
   {linear representation of group}%
\Index{texCartesian}%Л%116
   {лифт отображения}%
   {lift of map}%
\Index{texBundleRelation}%Л%232
   {лифт соответствия}%
   {lift of correspondence}%
\Index{texReferenceFrame}%Л%117
   {локальная система отсчёта}%
   {local reference frame}%
\SetIndexSpace%
\Index{texTstarRepresentation}%М%343
   {малая группа}%
   {little group}%
\Index{texDrcMorphism}%М%118
   {матрица \drc линейного отображения}%
   {matrix of drc linear map}%
\Index{texAffine}%М%119
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index{texDrcBasis}%М%120
   {многообразие базисов}%
   {}%
\SubIndex{texDrcBasis}%24%
   {\drc векторного пространства}%
   {basis manifold of vector space}%
\SubIndex{texTypeBasis}%25%
   {аффинного пространства}%
   {Basis Manifold, Affine Space}%
\SubIndex{texTypeBasis}%26%
   {евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\SubIndex{texTypeBasis}%27%
   {центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texBasis}%М%276
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index{texBasis}%М%268
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index{texBasis}%М%282
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index{texBasis}%М%280
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texReferenceFrame}%М%123
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index{texTstarMorphism}%М%298
   {морфизм \Ts представлений $\mathcal{F}$\Hyph алгебры}%
   {morphism of representations of F algebra}%
\Index{texTstarMorphism}%М%300
   {морфизм \Ts представлений $\mathcal{F}$\Hyph алгебры в $\mathcal{H}$\Hyph алгебре}%
   {morphism of representations of F algebra in H algebra}%
\Index{texTstarMorphism}%М%307
   {морфизм \Ts представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\SetIndexSpace%
\Index{texVectorSpace}%Н%124
   {невырожденная система \drc линейных уравнений}%
   {nonsingular system of linear equations}%
\Index{texRepresentation}%Н%241
   {невырожденное \Ts преобразование}%
   {nonsingular transformation}%
\Index{texReferenceFrame}%Н%125
   {неголономная координата}%
   {anholonomic coordinate}%
\Index{texReferenceFrame}%Н%126
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index{texReferenceFrame}%Н%127
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index{texAffine}%Н%128
   {неметричность}%
   {nonmetricity}%
\Index{texBundleRelation}%Н%339
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index{texCalculus}%Н%97
   {норма на \drc векторном пространстве}%
   {norm on drc vector space}%
\Index{texCalculus}%Н%100
   {норма на теле}%
   {absolute value on skew field}%
\Index{texCalculus}%Н%102
   {нормированное тело}%
   {valued skew field}%
\Index{texCalculus}%Н%104
   {нормированным \drc векторное пространство}%
   {normed drc vector space}%
\SetIndexSpace%
\Index{texBundleRelation}%О%121
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index{texBundleRelation}%О%115
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index{texBiring}%О%129
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index{texReferenceFrame}%О%130
   {объект неголономности}%
   {anholonomity object}%
\Index{texTstarRepresentation}%О%131
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texRepresentation}%О%259
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texFiberedGroup}%О%132
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index{texTstarMorphism}%О%303
   {однотранзитивное представление алгебры $A$}%
   {single transitive representation of algebra}%
\Index{texRepresentation}%О%258
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index{texFiberedAlgebra}%О%323
   {однотранзитивное представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {single transitive representation of fibered F-algebra}%
\Index{texFiberedAlgebra}%О%133
   {операция на расслоении}%
   {operation on bundle}%
\Index{texBiring}%О%134
   {определитель матрицы}%
   {determinant}%
\Index{texTstarRepresentation}%О%135
   {орбита \Ts представления группы}%
   {orbit of representation of group}%
\Index{texRepresentation}%О%253
   {орбита представления группы}%
   {orbit of representation of group}%
\Index{texFiberedGroup}%О%136
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index{texBasis}%О%281
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index{texTidal}%О%137
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index{texReferenceFrame}%О%138
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\SetIndexSpace%
\Index{texReferenceFrame}%П%139
   {параллелограмм}%
   {parallelogram}%
\Index{texTstarRepresentation}%П%140
   {парные представления группы}%
   {twin representations of group}%
\Index{texFiberedGroup}%П%319
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index{texLinearMap}%П%320
   {парные представления тела}%
   {twin representations of skew field}%
\Index{texDrcBasis}%П%141
   {пассивное \Ts представление}%
   {passive representation}%
\Index{texBasis}%П%273
   {пассивное представление}%
   {passive representation}%
\Index{texBasis}%П%272
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index{texNewton}%П%142
   {первый закон Ньютона}%
   {First Newton law}%
\Index{texAffine}%П%143
   {перенос Картана}%
   {Cartan transport}%
\Index{texAffine}%П%144
   {перенос Френе}%
   {Frenet transport}%
\Index{texBundleRelation}%П%220
   {подрасслоение}%
   {subbundle}%
\Index{texNewton}%П%146
   {потенциальная энергия}%
   {potential energy}%
\Index{texVectorSpace}%П%149
   {правое векторное пространство}%
   {right vector space}%
\Index{texLie}%П%151
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index{texRepresentation}%П%248
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation}%
\Index{texRepresentation}%П%250
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation}%
\Index{texTstarMorphism}%П%304
   {правостороннее представление $\mathcal{F}$\Hyph алгебры $A$ в множестве $M$}%
   {right-side representation of algebra}%
\Index{texRepresentation}%П%245
   {правостороннее представление группы}%
   {right-side representation of group}%
\Index{texFiberedAlgebra}%П%324
   {правостороннее представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {right-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%П%242
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texRepresentation}%П%243
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texLie}%П%153
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index{texVectorSpace}%П%215
   {правый модуль}%
   {right module}%
\Index{texTstarRepresentation}%П%158
   {правый сдвиг}%
   {right shift}%
\Index{texRepresentation}%П%252
   {правый сдвиг на группе}%
   {right shift, group}%
\Index{texBundleRelation}%П%342
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index{texBundleRelation}%П%335
   {предел фильтра}%
   {limit of filter}%
\Index{texBundleRelation}%П%334
   {предельное множество фильтра}%
   {limit set of filter}%
\Index{texBasis}%П%292
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texDrcBasis}%П%159
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texTstarRepresentation}%П%161
   {представление группы}%
   {}%
\SubIndex{texDrcBasis}%38%
   {\drc линейное \sT}%
   {linear representation of group}%
\SubIndex{texDrcBasis}%39%
   {\rcd}%
   {rcd linear representation of group}%
\SubIndex{texTstarRepresentation}%40%
   {\sT}%
   {starT representation of group}%
\SubIndex{texTstarRepresentation}%41%
   {\Ts}%
   {Tstar representation of group}%
\SubIndex{texTstarRepresentation}%42%
   {ковариантное \Ts}%
   {Tstar covariant representation of group}%
\SubIndex{texTstarRepresentation}%43%
   {контравариантное \Ts}%
   {Tstar contravariant representation of group}%
\SubIndex{texTstarRepresentation}%44%
   {эффективное}%
   {effective representation of group}%
\Index{texRepresentation}%П%246
   {представление группы}%
   {representation of group}%
\Index{texGenRelativity}%П%165
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index{texTstarMorphism}%П%313
   {преобразование множества}%
   {transformation of set}%
\Index{texDrcBasis}%П%166
   {преобразование на многообразии базисов}%
   {}%
\SubIndex{texDrcBasis}%62%
   {активное}%
   {active transformation, vector space}%
\SubIndex{texTypeBasis}%63%
   {аффинное}%
   {affine transformation}%
\SubIndex{texTypeBasis}%64%
   {движение}%
   {movement transformation}%
\SubIndex{texTypeBasis}%65%
   {квазиаффинное}%
   {quasi affine transformation}%
\SubIndex{texTypeBasis}%66%
   {квазидвижение}%
   {quasi movement}%
\SubIndex{texDrcBasis}%67%
   {пассивное}%
   {passive transformation, vector space}%
\Index{texFiberedAlgebra}%П%329
   {преобразование расслоения}%
   {transformation of bundle}%
\Index{texCartesian}%П%221
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index{texCartesian}%П%222
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index{texBundleRelation,texBundleRelation}%П%225
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index{texBundleRelation}%П%226
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index{texBiring}%П%168
   {приводимое бикольцо}%
   {reducible biring}%
\Index{texBiring}%П%169
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index{texBiring}%П%170
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index{texDrcBasis}%П%171
   {принцип инвариантности}%
   {invariance principle}%
\Index{texBasis}%П%296
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index{texBundleRelation}%П%235
   {продолжение соответствия}%
   {extension of correspondence}%
\Index{texDrcBasis}%П%173
   {произведение геометрического объекта и константы}%
   {product of geometrical object and constant}%
\Index{texBasis}%П%295
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometrical object and constant, vector space}%
\Index{texTstarMorphism}%П%299
   {произведение морфизмов \Ts представлений $\mathcal{F}$\Hyph алгебры}%
   {product of morphisms of representations of F algebra}%
\Index{texBundleRelation}%П%154
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index{texBundleRelation}%П%188
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\SubIndex{texVectorSpace}%74%
   {\drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\SubIndex{texVectorSpace}%75%
   {\rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index{texAffine}%П%174
   {производная Картана}%
   {Cartan derivative}%
\Index{texDiffProperty}%П%175
   {производная Ли}%
   {Lie derivative}%
\SubIndex{texDiffProperty}%72%
   {метрики}%
   {Lie derivative of metric}%
\SubIndex{texDiffProperty}%73%
   {связности}%
   {Lie derivative of connection}%
\Index{texTstarRepresentation}%П%352
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index{texCartesian}%П%333
   {пространство отображений}%
   {mapping space}%
\Index{texBundleRelation}%П%236
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index{texLieRepresentation}%П%177
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index{texTstarRepresentation}%П%178
   {прямое произведение \Ts представлений группы}%
   {direct product of representations of group}%
\Index{texRepresentation}%П%254
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index{texFiberedGroup}%П%179
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index{texReferenceFrame}%П%182
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index{texVectorSpace}%Р%183
   {размерность \drc векторного пространства}%
   {dimension of vector space}%
\Index{texFiberedMorphism}%Р%350
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index{texFiberedMorphism}%Р%349
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index{texFiberedAlgebra}%Р%184
   {расслоенная $\mathcal{F}$\Hyph алгебра}%
   {fibered F-algebra}%
\Index{texFiberedAlgebra}%Р%186
   {расслоенная $\mathcal{F}$\Hyph подалгебра}%
   {fibered F-subalgebra}%
\Index{texFiberedAlgebra}%Р%185
   {расслоенная группа}%
   {fibered group}%
\Index{texFiberedMorphism}%Р%347
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index{texFiberedMorphism}%Р%346
   {расслоенная малая группа}%
   {fibered little group}%
\Index{texBundleRelation}%Р%145
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index{texBundleRelation}%Р%237
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index{texBundleRelation}%Р%238
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index{texFiberedAlgebra}%Р%187
   {расслоенное кольцо}%
   {fibered ring}%
\Index{texBundleRelation}%Р%219
   {расслоенное подмножество}%
   {fibered subset}%
\Index{texBundleRelation}%Р%224
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index{texBundleRelation}%Р%330
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index{texBundleRelation}%Р%223
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index{texFiberedMorphism}%Р%337
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index{texFiberedMorphism}%Р%338
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index{texBundleRelation}%Р%157
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\SetIndexSpace%
\Index{texTstarRepresentation}%С%345
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index{texFiberedMorphism}%С%348
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index{texAffine}%С%189
   {связность Картана}%
   {Cartan connection}%
\Index{texAffine}%С%190
   {символ Картана}%
   {Cartan symbol}%
\Index{texBiring}%С%191
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index{texBundleRelation}%С%148
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index{texGenRelativity}%С%192
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index{texVectorSpace}%С%193
   {система \drc линейных уравнений}%
   {system of linear equations}%
\Index{texGenRelativity}%С%194
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index{texReferenceFrame}%С%195
   {система отсчёта на многообразии}%
   {reference frame}%
\Index{texNewton}%С%196
   {скалярный потенциал}%
   {scalar potential}%
\Index{texTidal}%С%197
   {скорость отклонения}%
   {speed of deviation}%
\Index{texBundleRelation}%С%297
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index{texBundleRelation}%С%340
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index{texBiring}%С%198
   {стандартное представление матрицы}%
   {Standard representation}%
\Index{texDrcBasis}%С%199
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBasis}%С%269
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBundleRelation}%С%234
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index{texLinearMap}%С%200
   {сумма \drc линейных отображений}%
   {sum of drc linear maps, drc vector spaces}%
\Index{texDrcBasis}%С%201
   {сумма геометрических объектов}%
   {sum of geometrical objects}%
\Index{texBasis}%С%294
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometrical objects, vector space}%
\SetIndexSpace%
\Index{texNewton}%Т%202
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index{texLie}%Т%203
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index{texVectorSpace}%Т%204
   {тип векторного пространства}%
   {vector space type}%
\Index{texReferenceFrame}%Т%205
   {типа $G$ система отсчёта}%
   {type G reference frame}%
\Index{texCalculus}%Т%152
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index{texCalculus}%Т%33
   {топологическое тело}%
   {topological skew field}%
\Index{texBundleRelation}%Т%147
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index{texTstarMorphism}%Т%305
   {транзитивное представление алгебры $A$}%
   {transitive representation of algebra}%
\Index{texRepresentation}%Т%257
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index{texFiberedAlgebra}%Т%325
   {транзитивное представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {transitive representation of fibered F-algebra}%
\SetIndexSpace%
\Index{texDiffProperty}%У%206
   {уравнение Килинга}%
   {Killing equation}%
\Index{texDiffProperty}%У%207
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index{texBiring}%У%208
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index{texFiberedMorphism}%Ф%336
   {фактор расслоение}%
   {quotient bundle}%
\Index{texBundleRelation}%Ф%341
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index{texCalculus}%Ф%150
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index{texCalculus}%Ф%68
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index{texBasis}%Ц%279
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index{texCalculus}%Ч%106
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, skew field}%
\Index{texCalculus}%Ч%107
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, drc vector space}%
\SetIndexSpace%
\Index{texAffine}%Э%209
   {экстремальная кривая}%
   {extreme line}%
\Index{texTstarMorphism}%Э%306
   {эффективное представление алгебры $A$}%
   {effective representation of algebra}%
\Index{texRepresentation}%Э%256
   {эффективное представление группы}%
   {effective representation of group}%
\Index{texFiberedAlgebra}%Э%326
   {эффективное представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {effective representation of fibered F-algebra}%
\Index{texFiberedGroup}%Э%315
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index{texVectorSpace}%Э%210
   {эффективное представление тела}%
   {effective representation of skew field}%
\SetIndexSpace%
\Index{texTstarRepresentation}%Я%211
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of representation of group}%
\Index{texRepresentation}%Я%255
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index{texFiberedGroup}%Я%212
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%

\CloseIndex


==> Preface.Algebra.Russian.tex <==
%auto-ignore
\def\texPreface_Algebra{}
\ifx\texPrefaceRelation\Defined
\ifx\PrintBook\Defined
				\chapter{Предисловие}
%\else
%			\section{Предисловие}
\fi
\epigraph{Кто-то из посетителей Ясной Поляны обвинил Толстого в том,
что он жестоко поступил с Анной Карениной
заставив ее броситься под поезд.
//
Толстой улыбнулся и ответил:
//
- Это мнение
напоминает мне случай с Пушкиным. Однажды он сказал
кому-то из своих приятелей: «Представь, какую штуку удрала со мной Татьяна.
Она замуж вышла. Этого я никак не ожидал от нее». То же самое и я могу сказать
про Анну Каренину. Вообще герои и героини мои делают иногда такие штуки, каких я
не желал бы! Они делают то, что должны делать в действительной жизни и
как бывает в действительной жизни, а не то, что мне хочется.}
{\citeBib{Tolstoi about Anna Karenina}, с. 517}
\fi

\ifx\texPrefaceAlgebra\Defined
Теория представления алгебры имеет длинную и богатую историю.
На протяжении XX столетия теория представления стала неотъемлемой частью многих
приложений. Переход от алгебры к расслоенной алгебре открывает новые возможности.
Я предпринял попытку написать эту
\ifx\PrintBook\Defined
книгу
\else
статью
\fi
с целью увидеть новые свойства
расслоенной алгебры.
\fi

\ifx\texPrefaceRelation\Defined
Эта история началась много лет назад. В 15 лет у меня появились карманные деньги на
расход.
Я стал покупать книги по математике и физике. К тому моменту,
когда я поступил в университет, я собрал библиотеку любимых книг.
Среди этих книг была книга "Универсальная алгебра" Кона
(\citeBib{Cohn: Universal Algebra}),
которая чудом задержалась в магазине. Я не очень задумывался, что мне
ещё рано читать об этом. Читая эту книгу я полюбил алгебру.
Однако свою жизнь и исследование я посвятил геометрии, работая
на стыке геометрии и физики.

Спустя более чем 30 лет, я вдруг вернулся к этой книге. Мне стало любопытно,
что будет, если универсальная алгебра определена в слое расслоения.
Когда я начал писать статью \citeBib{0702.561} меня не покидало
ощущение, что нечто подобное я читал в молодости. Я разыскал книгу,
которая, как я полагал, была первоисточником. Но в этой книге были только
векторные расслоения. Но лишь, когда я начал писать эту статью, я окончательно
понял, что ничего подобного я не читал. Я не смог бы пройти мимо подобных фактов.

Выходит, что в молодости я об этом думал. Но почему я ждал столько лет?
И почему именно сейчас я начал это исследование? На первый вопрос я никогда
не найду ответа. А ответ на второй вопрос очень прост.
На протяжении многих лет я изучал систему отсчёта в общей теории относительности.
При этом меня интересовал не только классический случай, но и возможные отклонения
геометрии. Результаты, полученные в \citeBib{0702.561}, показали,
что в области моего исследования есть ещё много оставшихся без ответа вопросов.

Я планировал посвятить эту статью изучению
расслоенного отношения эквивалентности, так как оно представляет для меня
определённый интерес в будущем.
Однако необходимость дать чёткие формулировки вовлекла новые определения.
Дальше события приняли совершено не предсказуемый оборот.
Статья, которая планировалась быть предельно короткой
и занять месяц работы, безжалостно отнимает у меня время, меняет название
и направление исследования.\footnote{Азарт
охоты - одна из самых сильных страстей человечества.
Я ловлю себя на том, что я постоянно решаю новые для меня задачи.}
Статья, посвящённая расслоенному отношению эквивалентности, превращается в статью,
посвящённую расслоенным бинарным отношениям.

Расслоенное отношение - пожалуй одна из самых тонких тем в теории расслоенной
алгебры. Определение операции практически однозначно переносится на расслоения, так как
операция является отображением, и относительно нетрудно распространить операцию на сечения
и, если надо, потребовать непрерывность. Отношение - это подмножество
декартового произведения.
Если мы просто определим его послойно, то скорее всего мы потеряем связь между слоями.

Я решил полностью повторить путь, который необходим для определения отношения в
универсальной алгебре.
Когда я начал изучать расслоенные соответствия, я понял, что многие
формулировки в \citeBib{0702.561} должны быть изменены.
Определение
\xRef{0702.561}{definition: reduced Cartesian product of bundle}
порождает слишком тесные рамки
для определения расслоенных соответствий.
Определение, задающее соответствие только в слое, может и хорошо в некоторых
случаях\footnote{В частности, мы определяем расслоенное отношение,
определяя отношение в слое}, но за бортом остаются
расслоенные морфизмы. Анализ сложившейся ситуации разоблачает миф, с которым
я спокойно жил все годы. Точнее, я всегда пытался понять,
что из себя представляет база послойного отображения.
Является ли это отображение инъекцией, или оно
может быть произвольным. Ни одно определение
не даёт ясного ответа на этот вопрос. Для простоты восприятия я полагал, что
база послойного отображения
является инъекцией. На самом деле, раз характер отображения базы не оговорен,
это отображение может быть произвольным. Это приводит к более широкому
определению (определение
\xRef{0702.561}{definition: Cartesian product of bundle}) декартова произведения расслоений.
С другой стороны, определение
\xRef{0702.561}{definition: Cartesian product of bundle} приводит к
трудностям в определении расслоенных алгебр. Это приводит к необходимости
пользоваться двумя определениями декартова произведения расслоения.
Аналогичные соображения приводят к двум определениям расслоенного соответствия.

В конце концов я вернулся к отношению эквивалентности. Но мой труд
не пропал даром. Мой взгляд на проблему изменился.

Из определения \ref{definition: Fibered Correspondence}
следует, что понятие непрерывности является существенной компонентой
определения расслоенного соответствия. Вслед за этим определением
я разъясняю, что означает непрерывность соответствия.
\fi

%В отличие от операций, отношения в расслоенной алгебре имеет меньше свойств.
%Тем не менее некоторые важные свойства сохраняются.
%Отношение эквивалентности играет большую роль в различных разделах математики.

\ifx\texPrefaceAlgebra\Defined
Так как сечения расслоения
может быть не определено на всём расслоении, все утверждения предполагают
некоторую область определения.
Подобные утверждения строятся по образцу утверждения
о существовании тривиального касательного расслоения на многообразии.

Однако существует другая группа утверждений, ограничивающих область
определения расслоенной
$\mathcal{F}$\Hyph алгебры. В тексте приведены соответствующие примеры.
Данная ситуация сводится к следующему.

Преобразование слоя при параллельном переносе предполагается
взаимно однозначным отображением.
Непрерывно перемещаясь вдоль базы,
мы непрерывно переходим от слоя к другому.
Предположение, что отображение между слоями является гомеоморфизмом,
гарантирует непрерывную деформацию слоя.

Если мы выберем точку в слое, то её траектория при движении проекции вдоль
базы будет параллельна базе. В дифференциальной
геометрии подобные кривые называются горизонтальными.
Мы так же будем придерживаться этого термина.

Если мы предполагаем на слое структуру
$\mathcal{F}$\Hyph алгебры, то соответствующее отображение
должно быть изоморфизмом $\mathcal{F}$\Hyph алгебры.
Непрерывность позволяет сохранить при параллельном переносе
изучаемые конструкции, сделать переход от слоя к слою
практически незаметным.

Эта картина хорошо работает в малом. Когда мы переходим к
конечным отрезкам на базе,
непрерывность становится ответственной за то,
что мы не можем продлить структуру $\mathcal{F}$\Hyph алгебры
сколь угодно далеко.
Например,  могут появиться точки, где гомеоморфизм может
быть нарушен. Это происходит, когда пересекаются горизонтальные кривые или
изменяются топологические свойства слоя. Соответствующий слой мы
называем вырожденным, а его проекцию - точкой вырождения.

Вопрос о том, как много точек вырождения, вообще говоря, непростой.
Интуитивно ясно, что это множество невелико по сравнению с базой.
Тем не менее, это множество может оказаться существенным
для изучения геометрии расслоения или физических процессов,
связанных с этим расслоением.

К подобным явлениям в теории дифференциальных уравнений
относится задача продления решения дифференциального уравнения.
В тоже время, дифференциальное уравнение может иметь два типа решения.
Регулярное решение принадлежит некоторому семейству
функций, зависящих от произвольных постоянных.
Особое решение является огибающей семейства регулярных решений.

Задача описания слоёв расслоения, независимо от того вырождены
они или нет, имеет интересное решение. Любой путь на базе расслоения
является отображением отрезка $I=[0,1]$ в базу расслоения.
Мы можем предположить, что слои расслоения не гомеоморфны,
но гомотопны.

Группа голономий расслоения также накладывает ограничение
на структуру расслоенной $\mathcal F$\Hyph алгебры
$\mathcal A=\bundle{}pA{}$. Естественно предположить, что при
параллельном переносе мы гомоморфно отображаем
$\mathcal F$\Hyph алгебру из одного слоя в другой.
Следовательно, предполагается, что преобразование, порождённое
параллельным переносом вдоль замкнутого контура
является гомоморфизмом $\mathcal F$\Hyph алгебры. Таким образом, всё хорошо,
если группа голономий расслоения $\mathcal A$ является
подгруппой группы гомоморфизмов $\mathcal F$\Hyph алгебры
$A$. В этом случае мы будем называть
расслоенную $\mathcal F$\Hyph алгебру $\mathcal A$
голономной.
В противном случае мы будем называть
расслоенную $\mathcal F$\Hyph алгебру $\mathcal A$
неголономной.

Из теории векторных расслоений известно, что не
не всякая расслоенная $\mathcal F$\Hyph алгебра
является голономной. В тоже время, теория векторных расслоений
предлагает рецепт каким образом мы можем работать с
неголономной расслоенной $\mathcal F$\Hyph алгеброй.

Это замечание относится также к теории представления
расслоенной $\mathcal F$\Hyph алгебры.

Чтобы сделать новые конструкции более наглядными,
я строю соответствующие диаграммы.
\fi

%Я следую соглашениям.
Обозначения операций и отношений по возможности
сохраняются как они введены в теории множеств. Это не приводит к
недоразумениям, так как обозначения расслоений отличны от обозначений
множеств. Для обозначения расслоения и слоя я буду пользоваться одной
и той же буквой в разных алфавитах.

Проекция расслоения, сечение, морфизм расслоений предполагаются непрерывными отображениями.

В математической литературе существует две традиции записывать произведение
отображений и соответствий. Одни авторы записывают произведение
отображений в том порядке, в каком стрелки следуют на диаграме.
Другие авторы предпочитают записывать отображения в противоположном
порядке. При чтении статей и книг надо первым делом обращать
внимание, какой порядок сомножителей использует автор.

Ситуация становится проще, когда автор записывает действие отображения
на множество. В этом случае автор записывает множество и отображение в таком
порядке, что расставив скобки, мы получим правильный порядок.
Например, рассмотрим диаграмму
\[
\xymatrix{
A\ar[r]^f&B\ar[r]^g&C
}
\]
и пусть $D\subset A$. Если мы произведение отображений записываем
в виде $fg$, то образ множества $D$ имеет вид $Dfg=(Df)g$.
Если мы произведение отображений записываем
в виде $gf$, то образ множества $D$ имеет вид $gfD=g(fD)$.

Это и является моей отправной точкой. Опираясь на соглашение
из замечания \xRef{0701.238}{remark: left and right matrix notation},
я буду предполагать возможность читать выражение как справа налево,
так и слева направо.

==> Relation.Russian.tex <==
%auto-ignore
\def\texBundleRelation{}

\ifx\PrintBook\Defined
				\chapter{Расслоенное отношение}

\fi

			\section{Соответствие}

		\begin{definition}
Пусть дана диаграмма
\[
\xymatrix{
A\ar[d]^\Phi\ar[rr]^\Psi&&B\ar[d]^\Sigma\\
C\ar[rr]^\Theta&&D
}
\]
стрелки которой изображают соответствия.
\AddIndex{Диаграмма соответствий}{diagram of correspondences} называется
\AddIndex{коммутативной}{commutative diagram of correspondences}, если образ любого подмножества
множества $A$ в множестве $D$ не зависит от пути в диаграмме.
		\qed
		\end{definition}

В определении категории мы не уточняем, является ли морфизм отображением.
Поэтому мы можем изучать категорию, объектами которой являются множества,
а морфизмами - соответствия из одного множества в другое.

		\begin{definition}
Пусть $\Phi$ - соответствие из множества $A$ в множество $B$.
Пусть $C\subseteq A$.
Мы будем говорить, что соответствие
\symb{\Phi/C}0{restriction of correspondence}
\[
\ShowSymbol{restriction of correspondence}=\{(c,b)\in\Phi:c\in C\}
\]
является \AddIndex{сужением соответствия $\Phi$ на множество $C$}
{restriction of correspondence}.\footnote{Определение
дано по аналогии с определением в \citeBib{Bourbaki: Set Theory}, с. 92}
Соответствие $\Phi$ называется \AddIndex{продолжением соответствия}
{extension of correspondence} $\Phi/C$.
		\qed
		\end{definition}

		\begin{definition}
		\label{definition: correspondence continuous on the set}
Предположим, что на множествах $A$ и $B$ определена топология.

Соответствие $\Phi$ из множества $A$ в множество $B$
называется
\AddIndex{непрерывным на множестве}{correspondence continuous on the set}
$C\subset A$,
если для любого открытого множества $V$,
$\Phi C\subset V\subset B$, существует открытое множество
$U$, $C\subset U\subset A$,
такое, что $\Phi U\subseteq V$.

Соответствие $\Phi$ из множества $A$ в множество $B$
называется \AddIndex{непрерывным}{continuous correspondence},
если для любого открытого множества
$V\subset B$ существует открытое множества $U\subset A$
такое, что $\Phi U\subseteq V$.
		\qed
		\end{definition}

Следуя \citeBib{Bourbaki: General Topology 1},
я определяю непрерывность, опираясь на понятие
предела по фильтру. Так как образ при соответствии является
не точкой, а множеством, определения и теоремы слегка изменены.

		\begin{definition}
		\label{definition: filter converges}
Пусть $X$ -  топологическое пространство. Пусть $\mathfrak{F}$ -
фильтр в $X$. Множество $A\subset X$ называют
\AddIndex{предельным множеством}{limit set of filter}
или \AddIndex{пределом фильтра}{limit of filter}
$\mathfrak{F}$, если $\mathfrak{F}$ мажорирует фильтр
$\mathfrak{B}(A)$ окрестностей множества $A$.
Говорят также, что фильтр $\mathfrak{F}$
\AddIndex{сходится}{filter converges} к $A$,
\symb{\mathfrak{F}\rightarrow A}1{filter converges}.

Множество $A$ называют пределом базиса фильтра $\mathfrak{B}$
в $X$ и говорят, что $\mathfrak{B}$ сходится к $A$,
если фильтр с базисом $\mathfrak{B}$ сходится к $A$.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: filter base converges to set}
Для того чтобы базис фильтра $\mathfrak{B}$ в топологическом
пространстве $X$ сходится к множеству $A\subset X$, необходимо
и достаточно, чтобы всякое множество из фундаментальной системы
окрестностей множества $X$ содержало множество из $\mathfrak{B}$.
		\end{theorem}
		\begin{proof} 
Если фильтр $\mathfrak{F}$ сходится к множеству $A$, то в силу
определения \ref{definition: filter converges} всякий фильтр,
мажорирующий $\mathfrak{F}$, также сходится к $A$.
Пусть $\Phi$ - множество фильтров в $X$, сходящихся к
множеству $A$. Так как фильтр окрестностей $\mathfrak{B}(A)$
мажорируется каждым фильтром из $\Phi$, то $\mathfrak{B}(A)$
мажорируется их пересечением $\mathfrak{G}$. Следовательно,
$\mathfrak{G}$ сходится к множеству $A$.
		\end{proof}

		\begin{definition}
		\label{definition: limit of correspondence with respect to the filter}
Пусть $\Phi$ - соответствие из множества $X$ в
топологическое пространство $Y$. Пусть $\mathfrak{F}\rightarrow A$ -
фильтр в $X$. Множество $B\subset Y$ называют
\AddIndex{пределом соответствия по фильтру}
{limit of correspondence with respect to the filter}
$\mathfrak{F}$
\symb{\lim_{\mathfrak{F}\rightarrow A}\Phi(\mathfrak{F})}
0{limit of correspondence with respect to the filter}
\[
\ShowSymbol{limit of correspondence with respect to the filter}=B
\]
если базис фильтра
$\Phi(\mathfrak{F})$ сходится к $B$.
		\qed
		\end{definition}

		\begin{theorem}
		\label{theorem: limit of correspondence}
Для того чтобы множество $B\subset Y$
было пределом соответствия $\Phi$ по фильтру
$\mathfrak{F}$, необходимо
и достаточно, чтобы для любой окрестности $V$ множества $B$
в $Y$ существовало такое множество $M\in\mathfrak{F}$,
что $\Phi M\subset V$.
		\end{theorem}
		\begin{proof} 
Следствие определения
\ref{definition: limit of correspondence with respect to the filter}
и теоремы \ref{theorem: filter base converges to set}.
		\end{proof}

		\begin{theorem}
		%\label{theorem: limit of correspondence}
Для того чтобы соответствия $\Phi$ из
топологического пространства $X$ в
топологическое пространство $Y$ было непрерывно
на множестве $A\subset X$, необходимо
и достаточно, чтобы
\[
\lim_{\mathfrak{F}\rightarrow A}\Phi(\mathfrak{F})=\Phi A
\]
		\end{theorem}
		\begin{proof} 
Следствие определения
\ref{definition: correspondence continuous on the set}
и теоремы \ref{theorem: limit of correspondence}.
		\end{proof}

Пусть $\Phi$ - непрерывное соответствие из
топологического пространства $X$ в
топологическое пространство $Y$. Пусть
$(a,b)\in\Phi$. Положим $V\subset Y$ - открытое множество,
$\Phi\{a\}\subset V$. В частности, $b\in V$.
Согласно определению
\ref{definition: correspondence continuous on the set}
существует открытое множество $U\subset X$, $a\in U$,
$\Phi U\subset V$. Следовательно, существуют $a'\in U$,
$b'\in V$, $(a',b')\in\Phi$.

			\section{Расслоенное соответствие}

		\begin{definition}
		\label{definition: fibered subset}
Пусть $\bundle{\mathcal{A}}aAN$ и $\bundle{\mathcal{B}}bBM$ - расслоения.
Пусть морфизм расслоений определён диаграммой
	\[
\xymatrix{
\mathcal{A}\arp[d]^{\bundle{}aA{}}\ar[rr]^f
&&\mathcal{B}\arp[d]^{\bundle{}{b}{B}{}}\\
N\ar[rr]^F&&M
}
	\]
где отображения $f$ и $F$ инъективны. Тогда мы называем расслоение $\bundle{}aA{}$
\AddIndex{расслоенным подмножеством}{fibered subset} или
\AddIndex{подрасслоением}{subbundle} расслоения $\bundle{}bB{}$.
Мы будем также пользоваться записью
\symb{\bundle{}{a}{A}{}\subseteq\bundle{}{b}{B}{}}1{fibered subset} либо
\symb{\mathcal{A}\subseteq\mathcal{B}}1{subbundle}.

Если на множествах $A$ и $B$ определена $\mathcal{F}$\Hyph алгебра и отображение $f$
является гомоморфизмом расслоенных алгебр, то расслоение $\bundle{}aA{}$
называется расслоенной подалгеброй расслоенной алгебры $\bundle{}bB{}$.
		\qed
		\end{definition}

Не нарушая общности, мы можем полагать $A\subseteq B$, $N\subseteq M$.

		\begin{definition}
		\label{definition: Fibered Correspondence}
Пусть $\bundle{\mathcal{A}}aAM$ и $\bundle{\mathcal{B}}bBN$ - расслоения.
Расслоенное подмножество $\bundle{\mathcal{F}}fF\Phi$ расслоения $\mathcal{A}\times\mathcal{B}$
называется \AddIndex{расслоенным соответствием из $\mathcal{A}$ в $\mathcal{B}$}{fibered correspondence from A to B}.

Если $\mathcal{A}=\mathcal{B}$, расслоенное соответствие $\mathcal{F}$ называется
\AddIndex{расслоенным соответствием в $\mathcal{A}$}{fibered correspondence in A}.
		\qed
		\end{definition}

Согласно определениям \ref{definition: fibered subset} и
\ref{definition: Fibered Correspondence}
расслоенное соответствие может быть
представлено с помощью диаграммы
\begin{equation}
\label{eq: Fibered Correspondence, definition}
\xymatrix{
\mathcal{F}\ar[rr]^j\arp[dd]^{\bundle{}fF{}}&&
\mathcal{A}\times\mathcal{B}
\arp@/^1pc/[dd]^{\bundle{}bB{}}
\arp@/_1pc/[dd]_{\bundle{}aA{}}\\
&&\times\\
\Phi\ar[rr]^i&&M\times N
}
\end{equation}
где $i$ и $j$ - непрерывные инъекции.
Мы полагаем, что множество $U\subset\Phi$ открыто тогда
и только тогда, когда существует открытое множество
$V\subset M\times N$ такое, что $U=V\cap\Phi$.
Мы полагаем, что множество $\mathcal{U}\subset\mathcal{F}$
открыто тогда
и только тогда, когда существует открытое множество
$\mathcal{V}\subset\mathcal{A}\times\mathcal{B}$
такое, что $\mathcal{U}=\mathcal{V}\cap\mathcal{F}$.

Мы будем называть соответствие $\Phi$
\AddIndex{базой расслоенного соответствия}{base of fibered correspondence}
$\mathcal{F}$, и расслоенное соответствие $\mathcal{F}$
мы будем называть \AddIndex{лифтом соответствия}{lift of correspondence} $\Phi$.

Мы будем пользоваться диаграммами расслоенных соответствий также,
как мы пользуемся диаграммами отображений и соответствий.
При этом мы можем дополнительно указать на диаграмме
проекцию на базу.
Таким образом расслоенное соответствие может быть
так же представлено с помощью диаграммы
\shorthandoff{"}
\begin{equation}
\label{eq: Fibered Correspondence, representation}
\xymatrix{
\mathcal{A}\ar[rr]^{\bundle{}pF{}}="AR1"\arp[d]^a&&\mathcal{B}\arp[d]^b\\
M\ar[rr]_f="AR2"&&N\\
\arp^{\bundle{}pF{}} "AR1";"AR2"
}
\end{equation}%
\shorthandon{"}%
Выбор диаграммы \eqref{eq: Fibered Correspondence, definition} или
\eqref{eq: Fibered Correspondence, representation}
будет зависеть от задачи, которую мы решаем.

Чтобы изучать расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$,
я буду пользоваться картами многообразий $M$ и $N$, в которых оба расслоения
тривиальны. Это позволит, не нарушая общности, в деталях изучить расслоенные
соответствия.

%Я дал столь общее определение, так как
%не хотел перегружать формулировку. В большинстве случаев повидимому достаточно
%потребовать, чтобы $F$ было отображением.

Согласно определению \xRef{0702.561}{definition: Cartesian product of bundle},
для произвольных $x\in M$, $y\in N$
точки слоя $(A\times B)_{(x,y)}$
расслоения $\mathcal{A}\times\mathcal{B}$ можно представить в
форме кортежа $(x,y,p,q)$, $p\in A_x$, $q\in B_y$. Согласно нашему допущению,
$\Phi\subseteq M\times N$, $F\subseteq A\times B$.
Следовательно, мы можем рассматривать $\Phi$ как соответствие из $M$ в $N$
и $F$ как соответствие из $A$ в $B$. В частности, $F_{(x,y)}\subseteq A_x\times B_y$.
Точка $(x,p)\in\mathcal{A}$ находится в соответствии $\mathcal{F}$ с точкой
$(y,q)\in\mathcal{B}$, если точка $x\in M$ находится в соответствии $\Phi$ с
точкой $y\in N$ и точка $p\in A_x$ находится в соответствии $F_{(x,y)}$ с
точкой $q\in B_y$.

Соответствие в слое зависит от выбора слоя. Например, пусть заданы
расслоения $\bundle{\mathcal{A}}aR{R^2}$ и $\bundle{\mathcal{B}}bRR$.
Пусть $(x,y)\in M=R^2$ и $z\in N=R$. Будем полагать, что точка
$(x,y,p)\in\mathcal{A}$ находится в соответствии $\mathcal{F}$
с точкой $(z,q)\in\mathcal{B}$, если $q$ можно представить в виде
\[
q=(z^2+x^2+y^2+p^2+1)n
\]
где $n$ - произвольное целое число. В разных слоях отношение
различно, однако мы можем определить биекцию между $F$ и $F_{(x,y,z)}$
для произвольного слоя.\footnote{Легко видеть, что небольшое изменение в
соответствии может привести к тому, что в некоторых
слоях соответствие будет вырождено.}

Рассмотрим множество $\Gamma(\mathcal{F})$. Если мы выберем
тривиализации расслоений $\mathcal{A}$ и $\mathcal{B}$, то
мы можем представить элемент $\Gamma(\mathcal{F})$ в виде
$(x,y,p(x),q(y))$. Небольшая перестановка элементов
приводит к записи $((x,p(x)),(y,q(y)))$. Возникает ощущение,
что мы записали соответствие из множества $\Gamma(\mathcal{A})$
в множество $\Gamma(\mathcal{B})$. Однако это не так.
Зафиксируем $x$. Тогда кортеж $(y,q(y))$ при изменении $y$
порождает сечение $q\in\Gamma(\mathcal{B})$. Так как это сечение
зависит от выбора пары $(x,p(x))$, то мы не можем установить
соответствия из множества $\Gamma(\mathcal{A})$
в множество $\Gamma(\mathcal{B})$.

Расслоенное соответствие
теряет некоторые важные свойства соответствия. Например,
если $C\subseteq A$ и $\Phi$ - соответствие из $A$ в $B$,
то мы можем определить образ множества $C$ при соответствии $\Phi$
с помощью равенства
\[
\Phi C=\{b\in B:(a,b)\in\Phi,a\in C\}
\]
Однако в случае расслоенного соотношения образ расслоения, вообще говоря,
расслоением не является. Причина состоит в том, что существует возможность,
что $(x_1,y)\in\Phi$, $(x_2,y)\in\Phi$. При этом, вообще говоря,
$$\Phi_{(x_1,y)}A_{x_1}\ne \Phi_{(x_2,y)}A_{x_2}$$ хотя
$$\Phi_{(x_1,y)}A_{x_1}\subseteq B_y$$ $$\Phi_{(x_2,y)}A_{x_2}\subseteq B_y$$
Следствием этого является невозможность определить в общем случае
произведение расслоенных соответствий.
Аналогичное утверждение справедливо для морфизмов расслоений, если база
морфизма не является инъекцией.

		\begin{theorem}
		\label{theorem: image of fibered correspondence}
Пусть определены расслоенное соответствие $\mathcal{F}$
\shorthandoff{"}
\[
\xymatrix{
\mathcal{A}\arp[d]^{\bundle{}pA{}}\ar[rr]^{\mathcal{F}}="AR1"
&&\mathcal{B}\arp[d]^{\bundle{}qB{}}\\
M\ar[rr]_f="AR2"&&N
\arp^{\bundle{}sF{}} "AR1";"AR2"
}
\]
\shorthandon{"}%
из расслоения $\mathcal{A}$ в расслоение $\mathcal{B}$,
база $f$ которого является инъекцией.
Пусть расслоение
\[\bundle{\mathcal{C}}aCL\]
является подрасслоением расслоения
$\mathcal{A}$. Мы определим образ
расслоение $\mathcal{C}$ при расслоенном соответствии $\mathcal{F}$
согласно равенству
\begin{align*}
\mathcal{F}\mathcal{C}=\{(y,b):&y\in N,\exists x\in M,y=f(x),\\
&b\in B_y,\exists a\in A_x,(a,b)\in F_{(x,y)}\}
\end{align*}
Образ расслоения $\mathcal{C}$ при расслоенном
соответствии $\mathcal{F}$
является подрасслоением расслоения $\mathcal{B}$.
		\end{theorem}
		\begin{proof}
Что бы доказать утверждение, мы должны показать, что все
$D_y=F_{(x,y)}C_x$ гомеоморфны.

Рассмотрим следующую диаграмму
\[
\xymatrix{
C_x\ar[dr]^{i_x}\ar[rrrr]^{F_{(x,y)}/C_x}\ar@{}[drrrr]|{(2)}&&&\ar@{}[dddr]|{(4)}&
D_y\ar[dl]_{j_y}&D_y=F_{(x,y)}C_x\\
&A_x\ar[rr]^{F_{(x,y)}}&&B_y&\\
&A\ar[rr]^F\ar[u]^l\ar@{}[urr]|{(5)}&&B\ar[u]^n&\\
C\ar[ur]^i\ar[uuu]^k\ar[rrrr]^{F/C}\ar@{}[uuur]|{(1)}\ar@{}[urrrr]|{(3)}&&&&
D\ar[ul]_j\ar[uuu]^m&D=FC
}
\]
$i$, $i_x$, $j$, $j_y$ - инъекции, $k$, $l$, $n$ - биекции.
Нам надо доказать, что $m$ - биекция. Мы предполагаем, что в
выбранном слое соответствие $F$ - не вырождено.

Биекция $l$ означает, что мы можем
перенумеровать точки множества $A_x$ точками множества $A$.
Биекция $k$ означает, что мы можем
перенумеровать точки множества $C_x$ точками множества $C$.
Инъекция $i$ означает, что $C\subseteq A$.
Инъекция $i_x$ означает, что $C_x\subseteq A_x$.
Следовательно, для каждой точки $p\in A$ однозначно определена точка $p_x\in A_x$.
Коммутативность диаграммы (1) означает, что
	\begin{equation}
p\in C\Leftrightarrow p_x\in C_x
	\label{eq: Fibered correspondence, p_x in C_x}
	\end{equation}

Биекция $n$ означает, что мы можем
перенумеровать точки множества $B_x$ точками множества $B$.
Инъекция $j$ означает, что $D\subseteq B$.
Инъекция $j_y$ означает, что $D_y\subseteq B_y$.
Следовательно, для каждой точки $q\in B$ однозначно определена точка $q_y\in B_y$.

Биекции $l$ и $n$ и коммутативность диаграммы (5) означает, что мы можем
перенумеровать точки соответствия $F_{(x,y)}$ точками соответствия
$F$\footnote{Требование невырожденности соответствия в слое
очень важно.
Если соответствие в слое будет вырождено,
то коммутативность диаграммы будет нарушена.}
	\begin{equation}
(p,q)\in F\Leftrightarrow (p_x,q_y)\in F_{(x,y)}
	\label{eq: Fibered correspondence, (p_x,q_y) in F_(x,y)}
	\end{equation}

По определению, $(p,q)\in F/C$, если $p\in C$ и $(p,q)\in F$.
Согласно \eqref{eq: Fibered correspondence, p_x in C_x} $p_x\in C_x$.
Согласно \eqref{eq: Fibered correspondence, (p_x,q_y) in F_(x,y)} $(p_x,q_y)\in F_{(x,y)}$.
По определению, $(p_x,q_y)\in F_{(x,y)}/C_x$.
Следовательно, $q_y\in D_y$, и отображение $m$ является инъекцией.
		\end{proof}

		\begin{theorem}
		%\label{theorem: image of fibered correspondence}
Пусть определены расслоенное соответствие $\bundle{}sF{}$
\[
\xymatrix{
\mathcal{A}\arp[d]^{\bundle{}pA{}}\ar[rr]^{\bundle{}sF{}}&&
\mathcal{B}\arp[d]^{\bundle{}qB{}}\\
M\ar[rr]^f&&N
}
\]
из расслоения $\mathcal{A}$ в расслоение $\mathcal{B}$
и расслоенное соответствие $\bundle{}tH{}$
\[
\xymatrix{
\mathcal{B}\arp[d]^{\bundle{}qB{}}\ar[rr]^{\bundle{}tH{}}&&
\mathcal{C}\arp[d]^{\bundle{}rC{}}\\
N\ar[rr]^h&&K
}
\]
из расслоения $\mathcal{B}$ в расслоение $\mathcal{C}$,
и базы расслоенных соответствий $\bundle{}sF{}$ и $\bundle{}tH{}$
являются инъекциями. Мы определим
\AddIndex{произведение расслоенных соответствий}
{composition of fibered correspondences}\footnote{Для соответствий
$\Phi$ и $\Psi$ произведение определено даже в том случае,
когда $\Phi$ - соответствие в множество $B$, а $\Psi$ - соответствие из
множества $C$. Однако мы не нарушим общности, если будем полагать,
что $\Phi$ - соответствие в множество $B\cap C$, а $\Psi$ - соответствие из
множества $B\cap C$. Это позволяет установить связь между
произведением соответствий и произведением расслоенных соответствий.}
$\mathcal{H}$ и $\mathcal{F}$
\symb{\bundle{}tH{}\circ\bundle{}sF{}}0{composition of fibered correspondences}
\begin{align*}
\ShowSymbol{composition of fibered correspondences}
=\{(x,z,a,c):&x\in M, z\in K,
\exists y\in N,y=f(x),z=h(y),\\
&a\in A_x, c\in C_z, \exists b\in B_y, (a,b)\in F_{(x,y)},(b,c)\in H_{(y,z)}\}
\end{align*}
		\end{theorem}
		\begin{proof}
Рассмотрим следующую диаграмму
\[
\xymatrix{
A_x\ar[rrrr]^{G_{(x,z)}}\ar[drr]^{F_{(x,y)}}\ar[ddd]^k&&&&C_z\ar[ddd]^l\\
&&B_y\ar[urr]^{H_{(y,z)}}\ar[d]^n&&\\
&&B\ar[drr]^H&&\\
A\ar[rrrr]^G\ar[urr]^F&&&&C
}
\]
$k$, $l$, $n$ - биекции.
Мы предполагаем, что в
выбранном слое соответствие $F$ - не вырождено.

Так же как и в доказательстве теоремы
\ref{theorem: image of fibered correspondence}
коммутативность вертикальных диаграмм означает, что
мы можем
перенумеровать точки соответствия $F_{(x,y)}$ точками соответствия $F$,
точки соответствия $H_{(y,z)}$ точками соответствия $H$,
точки соответствия $G_{(x,z)}$ точками соответствия $G$.

Коммутативность нижней диаграммы означает, что
$G=H\circ F$.
Коммутативность верхней диаграммы означает, что
$G_{(x,z)}=H_{(y,z)}\circ F_{(x,y)}$.
		\end{proof}

		\begin{theorem}
		\label{theorem: associative law, composition of fibered correspondences}
Пусть $\bundle{}sF{}$ - расслоенное соответствие
из расслоения $\mathcal{A}$ в расслоение $\mathcal{B}$,
$\bundle{}tH{}$ - расслоенное соответствие
из расслоения $\mathcal{B}$ в расслоение $\mathcal{C}$
и $\bundle{}rG{}$ - расслоенное соответствие
из расслоения $\mathcal{C}$ в расслоение $\mathcal{D}$.
Если определены произведения расслоенных соответствий
	\begin{equation}
\bundle{}tH{}\circ\bundle{}sF{}
	\label{eq: composition of fibered correspondences, F H}
	\end{equation}
и
	\begin{equation}
\bundle{}rG{}\circ\bundle{}tH{}
	\label{eq: composition of fibered correspondences, H G}
	\end{equation}
то так же определены произведения
$\bundle{}rG{}\circ(\bundle{}tH{}\circ\bundle{}sF{})$
и $(\bundle{}rG{}\circ\bundle{}tH{})\circ\bundle{}sF{}$.
В этом случае произведение расслоенных соответствий удовлетворяет
\AddIndex{закону ассоциативности}
{associative law, composition of fibered correspondences}
\[
\bundle{}rG{}\circ(\bundle{}tH{}\circ\bundle{}sF{})=
(\bundle{}rG{}\circ\bundle{}tH{})\circ\bundle{}sF{}
\]
		\end{theorem}
		\begin{proof}
Существование произведений
\eqref{eq: composition of fibered correspondences, F H} и
\eqref{eq: composition of fibered correspondences, H G} означает,
что база $f$ расслоенного соответствия $\bundle{}sF{}$,
база $h$ расслоенного соответствия $\bundle{}tH{}$ и
база $g$ расслоенного соответствия $\bundle{}rG{}$
являются инъекциями. При этом определены произведения отображений
$h\circ f$ и $g\circ h$, которые также являются инъекциями.
Следовательно, определены произведения отображений
$g\circ(h\circ f)$ и $(g\circ h)\circ f$, которые являются
инъекциями и удовлетворяют равенству
\[
g\circ(h\circ f)=(g\circ h)\circ f
\]
Следовательно, определено отображение базы расслоения $\mathcal{A}$ в
базу расслоения $\mathcal{D}$, и это отображение является инъекцией.

Существование произведений
\eqref{eq: composition of fibered correspondences, F H} и
\eqref{eq: composition of fibered correspondences, H G} означает,
что существует произведение соответствий $H\circ F$ и
$G\circ H$. Следовательно, существуют произведения соответствий
$G\circ(H\circ F)$ и $(G\circ H)\circ F$, которые удовлетворяют
закону ассоциативности. Следовательно, соответствие из слоя
расслоения $\mathcal{A}$ в слой
расслоения $\mathcal{D}$ определено однозначно.
		\end{proof}

		\begin{definition}
Пусть $\bundle{\mathcal{F}}sFf$ - расслоенное соответствие
\shorthandoff{"}
\[
\xymatrix{
\mathcal{A}\arp[d]^p\ar[rr]^{\mathcal{F}}="AR1"&&\mathcal{B}\arp[d]^q\\
M\ar[rr]_f="AR2"&&N
\arp^{\bundle{}sF{}} "AR1";"AR2"
}
\]
\shorthandon{"}%
из расслоения $\mathcal{A}$ в расслоение $\mathcal{B}$
и отображение $f$ является инъекцией.
Тогда определено
\AddIndex{обратное расслоенное соответствие}{inverse fibered correspondence}
\symb{\mathcal{F}^{-1}}0{inverse fibered correspondence, 1}
\symb{\bundle{}s{F^{-1}}{}}0{inverse fibered correspondence, 2}
$\bundle{\ShowSymbol{inverse fibered correspondence, 1}}s{F^{-1}}{f^{-1}}$
\shorthandoff{"}
\[
\xymatrix{
\mathcal{B}\arp[d]^p
\ar[rr]^{\ShowSymbol{inverse fibered correspondence, 1}}="AR1"
&&\mathcal{A}\arp[d]^q\\
N\ar[rr]_{f^{-1}}="AR2"&&M
\arp^{\ShowSymbol{inverse fibered correspondence, 2}} "AR1";"AR2"
}
\]
\shorthandon{"}%
	 \qed
	 \end{definition}

		\begin{definition}
Пусть $\bundle{\mathcal{A}}pAM$ - расслоение.
Расслоенное соответствие
\symb{\Delta_\mathcal{A}}0{diagonal in bundle, 1}
\symb{\bundle{}{r_\Delta}{\Delta_A}{}}0{diagonal in bundle, 2}
$$\bundle{\ShowSymbol{diagonal in bundle, 1}}{r_\Delta}{\Delta_A}{\Delta_M}$$
где проекция $\ShowSymbol{diagonal in bundle, 2}$ определена равенством
$$r_\Delta((x,p),(x,p))=(x,x)$$ называется
\AddIndex{диагональю в расслоении}{diagonal in bundle} $\mathcal{A}$.
		\qed
		\end{definition}

		\begin{theorem}
		%\label{theorem: image of fibered correspondence}
Пусть $\mathcal F$ - расслоенное соответствие
из расслоения $\mathcal{A}$ в расслоение $\mathcal{B}$,
$\mathcal H$ - расслоенное соответствие
из расслоения $\mathcal{B}$ в расслоение $\mathcal{C}$,
проекции расслоенных соответствий $\mathcal F$ и
$\mathcal H$ являются инъекциями.
Следующие тождества справедливы для
расслоенных соответствий $\mathcal F$ и
$\mathcal H$
\[
(\mathcal H\circ\mathcal F)^{-1}=\mathcal F^{-1}\circ\mathcal H^{-1}
\]
\[
(\mathcal F^{-1})^{-1}=\mathcal F
\]
\[
\mathcal F\circ\Delta_\mathcal{A}=\Delta_\mathcal{B}\circ\mathcal F=\mathcal F
\]
		\end{theorem}
		\begin{proof}
Доказательство теоремы аналогично доказательству теоремы
\ref{theorem: associative law, composition of fibered correspondences}.
Каждое утверждение проверяется на базе и в слое.
		\end{proof}

			\section{Расслоенное соответствие гомоморфизма}

Допустим функции перехода $f_{\alpha\beta}$ определяют расслоение
$\mathcal{A}$ над базой $M$.
Рассмотрим карты $U_\alpha\in M$ и $U_\beta\in M$, $U_\alpha\cap U_\beta\ne\emptyset$.
Точка $p\in\mathcal{A}$ имеет представление $(x,p_\alpha)$ в карте $U_\alpha$ и представление
$(x,p_\beta)$ в карте $U_\beta$.
Допустим функции перехода $g_{\epsilon\delta}$ определяют расслоение
$\mathcal{B}$ над базой $N$.
Рассмотрим карты $V_\epsilon\in N$ и $V_\delta\in N$,
$V_\epsilon\cap V_\delta\ne\emptyset$.
Точка $q\in\mathcal{B}$ имеет представление $(y,q_\epsilon)$ в карте $V_\epsilon$ и представление
$(y,q_\delta)$ в карте $V_\delta$.
Следовательно,
\[
p_\alpha=f_{\alpha\beta}(p_\beta)
\]
\[
q_\epsilon=g_{\epsilon\delta}(q_\delta)
\]
Представление соответствия при переходе от карты $U_\alpha$ к карте $U_\beta$
и от карты $V_\epsilon$ к карте $V_\delta$ изменяется согласно закону
\[
(x,y,p_\alpha,q_\epsilon)=(x,y,f_{\alpha\beta}(p_\beta),g_{\epsilon\delta}(q_\delta))
\]
Это согласуется с преобразованием
при переходе от карты $U_\alpha\times V_\epsilon$ к карте $U_\beta\times V_\delta$
в расслоении $\mathcal{A}\times\mathcal{B}$.

Это действительно необычный факт. Если на алгебре определена хоть одна операция,
уже достаточно потребовать, чтобы функции перехода были гомоморфизмами алгебры.
А здесь произвольные функции перехода, произвольное соответствие. И всё в порядке.

В отличие от операции единственное свойство, которое соответствие сохраняет,
- это принадлежность точки некоторому множеству. И до тех пор,
пока мы имеем дело с взаимно однозначными отображениями, нет оснований искать
ограничения на тип отображения. С другой стороны, операция в алгебре может
быть представлена в виде соответствия. Например, в векторном пространстве
мы можем рассмотреть соответствие вектора $a$ в вектор $b$ такое, что $a=3b$.
Линейное преобразование по определению сохраняет это соответствие. Что произойдёт
в случае нелинейного преобразования. Допустим мы применим преобразование координат
$a_i\rightarrow a_i^2$. Сохранится ли линейное отношение между векторами? Нет.
Сохранится ли само соответствие? Да, хотя выражено оно будет иначе. Векторы
остались те же, несмотря на изменение координат.

Отсюда вывод, что только в случае наложения на соответствие специальных ограничений,
мы накладываем ограничения на функции перехода.

		\begin{definition}
Соответствие $\Phi$ из $\mathcal{F}$\Hyph алгебры $A$ в $\mathcal{F}$\Hyph алгебру $B$
называется \AddIndex{соответствием гомоморфизма}
{correspondence of homomorphism},
если для каждой n\Hyph арной операции $\omega$ и любого
набора элементов $a_1$, ..., $a_n\in A$, $b_1$,
..., $b_n\in B$ таких, что
\[
(a_1,b_1)\in\Phi, ..., (a_n,b_n)\in\Phi
\]
справедливо
\[
(\omega(a_1,...,a_n),\omega(b_1,...,b_n))\in\Phi
\]
		\qed
		\end{definition}

		\begin{definition}
Соответствие $\Phi$ из $\mathcal{F}$\Hyph алгебры $A$ в $\mathcal{F}$\Hyph алгебру $B$
называется \AddIndex{расслоенным соответствием гомоморфизма}
{fibered correspondence of homomorphism},
если для каждой n\Hyph арной операции $\omega$ и любого
набора элементов $a_1$, ..., $a_n\in A$, $b_1$,
..., $b_n\in B$ таких, что
\[
(a_1,b_1)\in\Phi, ..., (a_n,b_n)\in\Phi
\]
справедливо
\[
(\omega(a_1,...,a_n),\omega(b_1,...,b_n))\in\Phi
\]
		\qed
		\end{definition}

			\section{Приведенное расслоенное соответствие}

		\begin{definition}
		\label{definition: reduced fibered correspondence}
Пусть $\bundle{\mathcal{A}}aAM$ и $\bundle{\mathcal{B}}bBM$ - расслоения над базой $M$.
Расслоенное подмножество $\bundle{\mathcal{F}}fFN$ расслоения $\mathcal{A}\odot\mathcal{B}$
называется \AddIndex{приведенным расслоенным соответствием из $\mathcal{A}$ в $\mathcal{B}$}
{reduced fibered correspondence from A to B}.

Если $\mathcal{A}=\mathcal{B}$, приведенное расслоенное соответствие $\mathcal{F}$ назывется
\AddIndex{приведенным расслоенным соответствием в $\mathcal{A}$}{reduced fibered correspondence in A}.
		\qed
		\end{definition}

Согласно определениям \ref{definition: fibered subset} и
\ref{definition: reduced fibered correspondence}
приведенное расслоенное соответствие может быть
представлено с помощью диаграммы
\begin{equation}
\label{eq: reduced fibered correspondence, definition}
\xymatrix{
\mathcal{F}\ar[rr]^j\arp[dd]_{\bundle{}fF{}}&&
\mathcal{A}\odot\mathcal{B}
\arp@/^1pc/[dd]^{\bundle{}bB{}}
\arp@/_1pc/[dd]_{\bundle{}aA{}}\\
&&\odot\\
M\ar[rr]^{\mathrm{id}}&&M
}
\end{equation}
где $j$ - непрерывная инъекция.
Мы полагаем, что множество $\mathcal{U}\subset\mathcal{F}$
открыто тогда
и только тогда, когда существует открытое множество
$\mathcal{V}\subset\mathcal{A}\odot\mathcal{B}$
такое, что $\mathcal{U}=\mathcal{V}\cap\mathcal{F}$.

Приведенное расслоенное отношение определено только для точек одного слоя.
Чтобы изучать приведенное расслоенное соответствие
из $\mathcal{A}$ в $\mathcal{B}$,
я буду пользоваться картами многообразия $M$, в которых оба расслоения
тривиальны. Это позволит, не нарушая общности, в деталях изучить
приведенные расслоенные
соответствия.

Согласно определению \xRef{0702.561}{definition: reduced Cartesian product of bundle},
точки слоя $(A\times B)_x$ расслоения $\mathcal{A}\odot\mathcal{B}$ можно представить в
форме кортежа $(x,p,q)$, $p\in A_x$, $q\in B_x$.
Точка $(x,p)\in\mathcal{A}$ находится в
приведенном расслоенном соответствии $\mathcal{F}$ с точкой
$(x,q)\in\mathcal{B}$, если $x\in N\subseteq M$
и точка $p\in A_x$ находится в соответствии $F_x$ с
точкой $q\in B_x$.
Следовательно, мы можем рассматривать $F_x$ как соответствие из $A_x$ в $B_x$.
В частности, $F_x\subseteq A_x\times B_x$.

Поскольку приведенное расслоенное соответствие наследует
топологию расслоения $\mathcal{A}\odot\mathcal{B}$,
то мы можем проанализировать какую роль играет топология
приведенного расслоенного соответствия.
Пусть точка $p\in A_x$ находится в соответствии $F_x$ с
точкой $q\in B_x$. Пусть
$\mathcal{V}\subset\mathcal{A}\odot\mathcal{B}$ -
открытое множество такое, что $(x,p,q)\in\mathcal{V}$.
Согласно \citeBib{Bourbaki: General Topology 1}, стр. 58,
существуют открытые множества $U\subset M$,
$V\subset A\times B$ такие, что
$x\in U$, $(p,q)\in V\cap F$.
Следовательно, существуют $x'\in U$,
$(p',q')\in V\cap F$.
Если $x\ne x'$, то мы можем выразить этот факт
как утверждение о непрерывной зависимости соответствия от слоя.
Однако из непрерывной зависимости соответствия от слоя не
следует непрерывность соответствия в слое. 

		\begin{theorem}
		\label{theorem: reduced fibered correspondence}
Для приведенного расслоенного соответствия $\bundle{\mathcal{F}}fFN$
однозначно определены расслоенное соответствие
$\bundle{\mathcal{F}}{f_\Delta}F{\Delta_N}$ - лифт диагонали $\Delta_N$
и изоморфизм расслоений
	\begin{equation}
\xymatrix{
\mathcal{F}\arp[d]^{\bundle{}{f_\Delta}F{}}\ar[rr]^{id}
&&\mathcal{F}\arp[d]^{\bundle{}fF{}}\\
\Delta_N\ar[rr]^{\pi}&&N
}
	\label{eq: Reduced Fibered correspondence}
	\end{equation}
над базой $\pi:\Delta_N\rightarrow N$.
		\end{theorem}
		\begin{proof}
Согласно построению, $F_{(x,x)}=F_x$.
		\end{proof}

Мы будем записывать диаграмму \eqref{eq: Reduced Fibered correspondence}
в более компактной форме
\[
\xymatrix{
&\mathcal{F}\arp[ld]_{\bundle{}{f_\Delta}F{}}
\arp[rd]^{\bundle{}fF{}}&\\
\Delta_N\ar[rr]^{\pi}&&N
}
\]
 
Теореме \ref{theorem: reduced fibered correspondence}
позволяет построить две категории:
\begin{itemize}
\item \AddIndex{категория приведенных расслоенных соответствий}
{category of reduced fibered correspondences},
объектами которой являются
расслоения над заданной базой и морфизмами которой являются
приведенные расслоенные соответствия
\item \AddIndex{категория расслоенных соответствий над диагональю}
{category of fibered correspondences over diagonal},
объектами которой являются
расслоения над заданной базой $M$ и морфизмами которой являются
расслоенные соответствия база, которых является диагональю в $M$
\end{itemize}
Функтор между этими категориями определён тривиальным образом. Он отображает
объекты и морфизмы в самих себя, однако в случае морфизмов проекция на базу
заменяется проекцией на диагональ.

	\begin{remark}
	\label{remark: base of reduced fibered correspondences}
Из вышеизложенного следует, что не нарушая общности мы можем
положить, что $N=M$. Так же как в
\ifx\PrintBook\Defined
замечании \ref{remark: reduce details on the diagram, algebra bundle}
\else
секции \xRef{0702.561}{section: Representation of Fibered F-Algebra}
\fi
мы можем не указывать базу на диаграмме приведенных расслоенных соотношений.
Согласно теореме \ref{theorem: reduced fibered correspondence}
для нас не имеет значение используем ли мы в качестве базы множество
$M$ или множество $\Delta_M$.
		\qed
	\end{remark}

Допустим функции перехода $f_{\alpha\beta}$ определяют расслоение
$\mathcal{A}$ над базой $M$
и функции перехода $g_{\alpha\beta}$ определяют расслоение $\mathcal{B}$
над базой $M$.
Рассмотрим на $M$ две карты $U_\alpha$ и $U_\beta$, $U_\alpha\cap U_\beta\ne\emptyset$.
Точка $p\in\mathcal{A}$ имеет представление $(x,p_\alpha)$ в карте $U_\alpha$ и представление
$(x,p_\beta)$ в карте $U_\beta$.
Точка $q\in\mathcal{B}$ имеет представление $(x,q_\alpha)$ в карте $U_\alpha$ и представление
$(x,q_\beta)$ в карте $U_\beta$.
Следовательно,
\[
p_\alpha=f_{\alpha\beta}(p_\beta)
\]
\[
q_\alpha=g_{\alpha\beta}(q_\beta)
\]
Представление соответствия при переходе от карты $U_\alpha$ к карте $U_\beta$
изменяются согласно закону
\[
(x,p_\alpha,q_\alpha)=(x,f_{\alpha\beta}(p_\beta),g_{\alpha\beta}(q_\beta))
\]
Это согласуется с законом преобразования
при переходе от карты $U_\alpha$ к карте $U_\beta$
в расслоении $\mathcal{A}\odot\mathcal{B}$.

		\begin{theorem}
Если определено приведенное
расслоенное соответствие $\mathcal{F}$ из $\mathcal{A}$ в $\mathcal{B}$,
то множество $\Gamma(\mathcal{F})$ определяет соответствие
из $\Gamma(\mathcal{A})$ в $\Gamma(\mathcal{B})$.
		\end{theorem}
		\begin{proof}
Согласно замечанию
\xRef{0702.561}{remark: reduced Cartesian product, section},
сечение расслоения $\mathcal{A}\odot\mathcal{B}$ можно представить в
форме кортежа $(f,g)$, где $f$ сечение расслоения $\mathcal{A}$
и $g$ сечение расслоения $\mathcal{B}$. В каждом слое $f(x)\in A_x$ находится в
соответствии $F$ с $g(x)\in B_x$ тогда и только тогда, когда сечение $(f,g)\in\Gamma(\mathcal{F})$.
		\end{proof}

Свойства приведенного расслоенного соответствия ближе к свойствам обычного соответствия.

		\begin{theorem}
Пусть определено приведенное расслоенное соответствие $\mathcal{F}$ из $\mathcal{A}$ в $\mathcal{B}$,
и расслоение $\mathcal{A'}\subseteq\mathcal{A}$. Мы определим образ
расслоение $\mathcal{A'}$ при приведенном соответствии $\mathcal{F}$
согласно равенству
\[
\mathcal{F}\mathcal{A}'=\{(x,b):x\in M,(a,b)\in F_x,a\in A_x\}
\]
Образ расслоения $\mathcal{A'}$ при приведенном
расслоенном соответствии $\mathcal{F}$
является подрасслоением расслоения $\mathcal{B}$.
		\end{theorem}
		\begin{proof}
Рассмотрим\footnote{Я могу слово в слово с точностью до обозначений повторить доказательство теоремы
\ref{theorem: image of fibered correspondence}. Однако я хочу привести другое доказательство,
чтобы показать как работает теорема \ref{theorem: reduced fibered correspondence}.}
коммутативную диаграмму расслоенных соответствий
	\begin{equation}
\xymatrix{
\mathcal{A}'\ar[d]^{F/A'}\ar[rr]^I&&
\mathcal{A}\ar[d]^F\\
\mathcal{B}'\ar[rr]^J&&\mathcal{B}
}
	\label{eq: image of reduced fibered correspondence}
	\end{equation}

В зависимости от выбранных проекций эта диаграмма представляет взаимодействие
приведенных расслоенных соответствий над базой $M$, либо
взаимодействие расслоенных соответствий над базой $\Delta_M$.
Однако это одни и те же соответствия. Все соотношения, справедливые для
базы $\Delta_M$, справедливы также для базы $M$.
		\end{proof}

	\begin{remark}
Диаграмма
\eqref{eq: image of reduced fibered correspondence} выглядит просто.
Однако, если мы её запишем без учёта замечания
\ref{remark: base of reduced fibered correspondences},
эта диаграмма примет вид
\[
\xymatrix{\\
\mathcal{A}'\ar[rr]^{F/A'}\ar@/^2pc/[rrrr]^I\arp@/_1pc/[dr]^{\bundle{}{p_\Delta}{A'}{}}
\arp@/_2pc/[ddr]_{\bundle{}p{A'}{}}&&
\mathcal{B}'\ar@/^2pc/[rrrr]^J\arp@/^1pc/[dl]_{\bundle{}{q_\Delta}{B'}{}}
\arp@/^2pc/[ddl]^{\bundle{}q{B'}{}}&&
\mathcal{A}\ar[rr]^F\arp@/_1pc/[dr]^{\bundle{}{r_\Delta}A{}}
\arp@/_2pc/[ddr]_{\bundle{}rA{}}&&
\mathcal{B}\arp@/^1pc/[dl]_{\bundle{}{s_\Delta}B{}}
\arp@/^2pc/[ddl]^{\bundle{}sB{}}\\
&\Delta_N\ar[d]\ar[rrrr]^{i_\Delta}&&&&\Delta_M\ar[d]\\
&N\ar[rrrr]^i&&&&M
}
\]
На диаграмме принято соглашение
\[
i_\Delta(a,a)=(i(a),i(a))
\]
		\qed
	\end{remark}

		\begin{theorem}
		\label{theorem: composition of reduced fibered correspondences}
Пусть определены приведенное расслоенное соответствие $\bundle{}sF{}$ из
расслоения $\mathcal{A}$ в расслоение $\mathcal{B}$
и приведенное расслоенное соответствие $\bundle{}tH{}$ из
расслоения $\mathcal{B}$ в расслоение $\mathcal{C}$.
Мы определим
\AddIndex{произведение приведенных расслоенных соответствий}
{composition of reduced fibered correspondences}
$\bundle{}sF{}$ и $\bundle{}tH{}$
\[
\bundle{}tH{}\circ\bundle{}sF{}=\{(x,a,c):x\in M,(a,b)\in F_x,(b,c)\in H_x\}
\]
		\end{theorem}
		\begin{proof}
Из коммутативности диаграммы расслоенных соответствий
\[
\xymatrix{
A_x\ar[dd]^{G_x}\ar[drr]^{F_x}&&&&&&A\ar[dd]^G\ar[dll]^F\ar[llllll]\\
&&B_x\ar[dll]^{H_x}&&B\ar[drr]^H\ar[ll]&&\\
C_x&&&&&&C\ar[llllll]
}
\]
над базой $\Delta_M$ следует $G_x=H_x\circ F_x$. Следовательно
это равенство справедливо также над базой $M$.
		\end{proof}

		\begin{definition}
		\label{definition: inverse reduced fibered correspondence}
Пусть $\bundle{\mathcal{F}}sFM$ - приведенное расслоенное соответствие
\[
\xymatrix{
\mathcal{A}\arp@/_1pc/[dr]_p\ar[rr]^{\mathcal{F}}&
\arp[d]^{\bundle{}sF{}}&\mathcal{B}\arp@/^1pc/[dl]^q\\
&M&
}
\]
%\shorthandoff{"}
%\POS"AR1"\ar[d]
%\ar @{.>}^{\bundle{}pF{}} "AR1";"N1"
%\shorthandon{"}%
из расслоения $\mathcal{A}$ в расслоение $\mathcal{B}$.
Тогда определено
\AddIndex{обратное приведенное расслоенное соответствие}
{inverse reduced fibered correspondence}
\symb{\mathcal{F}^{-1}}0{inverse reduced fibered correspondence, 1}
\symb{\bundle{}s{F^{-1}}{}}0{inverse reduced fibered correspondence, 2}
$\bundle{\ShowSymbol{inverse reduced fibered correspondence, 1}}s{F^{-1}}M$
\[
\xymatrix{
\mathcal{B}\arp@/_1pc/[drr]_p
\ar[rrrr]^{\ShowSymbol{inverse reduced fibered correspondence, 1}}&&
\arp[d]^{\ShowSymbol{inverse reduced fibered correspondence, 2}}&&
\mathcal{A}\arp@/^1pc/[dll]^q\\
&&M&&
}
\]
	 \qed
	 \end{definition}

		\begin{theorem}
Диагональ $\Delta_\mathcal{A}$ в расслоении $\bundle{\mathcal{A}}pAM$
является приведенным расслоенным соответствием
\symb{\bundle{}r{\Delta_A}{}}0{diagonal in reduced bundle, 2}
$$\ShowSymbol{diagonal in reduced bundle, 2}:\Delta_\mathcal{A}\rightarrow M$$
где проекция $\bundle{}r{\Delta_A}{}$ определена равенством
$$\bundle{}r{\Delta_A}{}(x,(p,p))=x$$
		\qed
		\end{theorem}

		\begin{theorem}
		%\label{theorem: image of fibered correspondence}
Пусть $\mathcal F$ - приведенное расслоенное соответствие
из расслоения $\mathcal{A}$ в расслоение $\mathcal{B}$,
$\mathcal H$ - приведенное расслоенное соответствие
из расслоения $\mathcal{B}$ в расслоение $\mathcal{C}$.
Следующие тождества справедливы для
приведенных расслоенных соответствий $\mathcal F$ и
$\mathcal H$
\[
(\mathcal H\circ\mathcal F)^{-1}=\mathcal F^{-1}\circ\mathcal H^{-1}
\]
\[
(\mathcal F^{-1})^{-1}=\mathcal F
\]
\[
\mathcal F\circ\Delta_\mathcal{A}=\Delta_\mathcal{B}\circ\mathcal F=\mathcal F
\]
		\end{theorem}
		\begin{proof}
Доказательство теоремы аналогично доказательству теоремы
\ref{theorem: associative law, composition of fibered correspondences}.
Каждое утверждение проверяется на базе и в слое.
		\end{proof}

			\section{Расслоенное отношение}
			\label{section: Fibered Relation}

	\begin{definition}
	\label{definition: Fibered Relation}
Пусть $\bundle{\mathcal{A}}pAM$ -
расслоение и $\omega$ - $n$\Hyph арное отношение в множестве $A$.
Расслоенное подмножество $\bundle{}r\omega{}$ расслоения
$\mathcal{E}^n$ называется \AddIndex{$n$\Hyph арным расслоенным отношением}
{fibered relation} в расслоении $\mathcal{A}$.
	 \qed
	 \end{definition}

		\begin{theorem}
		\label{theorem: 2 ary fibered relation}
\AddIndex{$2$\Hyph арное расслоенное отношение}
{2 ary fibered relation} в расслоении $\mathcal{A}$
является приведенным расслоенным соответствием в расслоении $\mathcal{A}$.
		\end{theorem}
		\begin{proof}
Теорема является следствием определений
\ref{definition: reduced fibered correspondence} и
\ref{definition: Fibered Relation}.
		\end{proof}

	\begin{definition}
%	\label{definition: Fibered Relation}
$2$\Hyph арное расслоенное отношение $\mathcal{F}$
в расслоении $\mathcal{A}$ называется
\begin{itemize}
\item \AddIndex{транзитивным}
{transitive 2 ary fibered relation}, если
$\mathcal{F}\circ\mathcal{F}\subseteq\mathcal{F}$
\item \AddIndex{симметричным}{symmetric 2 ary fibered relation},
если $\mathcal{F}^{-1}=\mathcal{F}$
\item \AddIndex{антисимметричным}{antisymmetric 2 ary fibered relation},
если $\mathcal{F}\cap\mathcal{F}^{-1}\subseteq\Delta_\mathcal{A}$
\item \AddIndex{рефлексивным}{reflexive 2 ary fibered relation},
если $\mathcal{F}\supseteq\Delta_\mathcal{A}$
\end{itemize}
	 \qed
	 \end{definition}

	\begin{definition}
Транзитивное рефлексивное $2$\Hyph арное расслоенное отношение $\mathcal{F}$
в расслоении $\mathcal{A}$ называется
\AddIndex{расслоенной предупорядоченностью}
{fibered preordering} в $\mathcal{A}$.
В этом случае $\mathcal{F}^{-1}$ также является
расслоенной предупорядоченностью в $\mathcal{A}$,
которая называется \AddIndex{противоположной}
{opposite fibered preordering} к $\mathcal{F}$.
Антисимметричная расслоенная предупорядоченность
в расслоении $\mathcal{A}$ называется
\AddIndex{расслоенной упорядоченностью}
{fibered ordering} в $\mathcal{A}$.\footnote{Было бы заманчиво
определить расслоенную линейную упорядоченность $\mathcal{F}$
с помощью равенства $$\mathcal{F}\cup\mathcal{F}^{-1}=
\mathcal{A}^2$$ Однако, если мы рассмотрим это отношение на множестве
сечений, то мы можем найти пару сечений, которые мы не можем сравнить.}
	 \qed
	 \end{definition}

	\begin{definition}
Транзитивное рефлексивное симметричное
$2$\Hyph арное расслоенное отношение $\mathcal{F}$
в расслоении $\mathcal{A}$ называется
\AddIndex{расслоенной эквивалентностью}
{fibered equivalence} на расслоении $\mathcal{A}$.
	 \qed
	 \end{definition}

%		\begin{theorem}
%Пусть $\mathcal{F}$ -
%$2$\Hyph арное расслоенное отношение в расслоении $\mathcal{A}$.
%Тогда на множестве $\mathcal{A}$ определенно соответствие $\Phi$
%такое, что 
%		\end{theorem}
%		\begin{proof}
%Теорема является следствием определений
%\ref{definition: reduced fibered correspondence} и
%\ref{definition: Fibered Relation}.
%		\end{proof}

Рассмотрим расслоенную эквивалентность $\mathcal{F}$ 
расслоении $\mathcal{A}$. Для каждого $x\in M$ в слое $A_x$ определено
отношение эквивалентности $F_x$.

==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant definition}%
\Symb{texBiring}%
   {минор}%
   {A from b a}%
\Symb{texBiring}%
   {минор}%
   {A from columns T}%
\Symb{texBiring}%
   {минор}%
   {A from rows S}%
\Symb{texBiring}%
   {минор}%
   {A without column a}%
\Symb{texBiring}%
   {минор}%
   {A without columns T}%
\Symb{texBiring}%
   {минор}%
   {A without row b}%
\Symb{texBiring}%
   {минор}%
   {A without rows S}%
\Symb{texPolymodule}%
   {активное преобразование}%
   {active transformation}%
\Symb{texTypeBasis}%
   {аффинное пространство}%
   {affine space}%
\Symb{texBasis}%
   {аффинное пространство}%
   {An}%
\Symb{texBiring}%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb{texBiring}%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb{texBiring}%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb{texBiring}%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb{texVectorSpace}%
   {\dcr вектор}%
   {dcr vector}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb{texVectorSpace}%
   {\drc вектор}%
   {drc vector}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb{texPolymodule}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texBiring}%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb{texBiring}%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb{texBiring}%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb{texBiring}%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb{texBiring}%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb{texTstarRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texFiberedGroup}%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb{texTstarRepresentation}%
   {левый сдвиг}%
   {Tstar shift}%
\Symb{texFiberedGroup}%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb{texReferenceFrame}%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb{texReferenceFrame}%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%
\Symb{texBasis}%
   {многообразие базисов аффинного пространства}%
   {BAn}%
\Symb{texReferenceFrame}%
   {многообразие базисов многообразия}%
   {basis manifold of manifold}%
\Symb{texPolymodule}%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства $\mathcal{V}$}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb{texBasis}%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb{texCartesian}%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb{texTypeBasis}%
   {многообразие базисов аффинного пространства}%
   {FAn}%
\Symb{texTypeBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb{texTypeBasis}%
   {многообразие базисов евклидова пространства}%
   {FEn}%

\SetIndexSpace%
\Symb{texBasis}%
   {центро-аффинное пространство}%
   {CAn}%
\Symb{texTypeBasis}%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb{texLie}%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb{texLie}%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb{texReferenceFrame}%
   {множество функций, определённых на многообразии}%
   {set of functions defined on manifold}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation, coordinates}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation, coordinates}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство \subs строк}%
   {c rows dcr vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to drc vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to skew field}%
\Symb{texVectorSpace}%
   {\drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Symb{texVectorSpace}%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace D}%
\Symb{texAffine}%
   {производная}%
   {overline D}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, skew field}%
\Symb{texVectorSpace}%
   {\drc векторное пространство \sups строк}%
   {r rows drc vector space}%
\Symb{texTidal}%
   {скорость отклонения}%
   {speed of deviation}%
\Symb{texVectorSpace}%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%
\Symb{texTypeBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texTypeBasis}%
   {базис}%
   {basis}%
\Symb{texBasis}%
   {базис векторного пространства}%
   {Basis e}%
\Symb{texBasis}%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb{texVectorSpace}%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb{texPolymodule}%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb{texCartesian}%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb{texBasis}%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb{texReferenceFrame}%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb{texTypeBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texTypeBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texFiberedAlgebra}%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb{texBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb{texBasis}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texReferenceFrame}%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb{texReferenceFrame}%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb{texReferenceFrame}%
   {векторное поле системы отсчёта}%
   {vector field, reference frame}%
\Symb{texBasis}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {координаты базиса в \dcr векторном пространстве \subs строк}%
   {basis coordinates, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {координаты базиса в \drc векторном пространстве \sups строк}%
   {basis coordinates, r rows drc vector space}%
\Symb{texVectorSpace}%
   {базис в \dcr векторном пространстве \subs строк}%
   {basis, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {базис в \drc векторного пространства \sups строк}%
   {basis, r rows drc vector space}%
\Symb{texDiffEq}%
   {центро-аффинный}%
   {Central Affine Basis}%
\Symb{texReferenceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Symb{texBundleRelation}%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb{texFiberedAlgebra}%
   {гомоморфизм расслоенных $\mathcal{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb{texCartesian}%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb{texTstarRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%
\Symb{texTypeBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texReferenceFrame}%
   {система отсчёта}%
   {reference frame}%
\Symb{texReferenceFrame}%
   {система отсчёта}%
   {reference frame, extensive definition}%
\Symb{texPolymodule}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texPolymodule}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb{texFiberedMorphism}%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb{texFiberedMorphism}%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb{texLie}%
   {алгебра Ли группы Ли}%
   {g}%
\Symb{texLie}%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb{texTypeBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texLie}%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb{texBasis}%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb{texTstarRepresentation}%
   {малая группа элемента $x$}%
   {little group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective starT covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective starT covariant representation of group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective Tstar covariant representation of group}%
\Symb{texVectorSpace}%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb{texTstarRepresentation}%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%
\Symb{texBiring}%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb{texLinearMap}%
   {\rcd векторное пространство \drc линейных отображений}%
   {rcd vector space of drc linear maps}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb{texLinearLie}%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%
\Symb{texRepresentation}%
   {левый сдвиг}%
   {left shift}%
\Symb{texDiffProperty}%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb{texDiffProperty}%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb{texBundleRelation}%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb{texBasis}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texRepresentation}%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texTstarMorphism}%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb{texTstarMorphism}%
   {множество \Ts преобразований множества $M$}%
   {set of Tstar transformations}%
\Symb{texTstarRepresentation}%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%
\Symb{texBasis}%
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Symb{texBasis}%
   {геометрический объект}%
   {geometrical object, vector space}%
\Symb{texFiberedGroup}%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of fibered group}%
\Symb{texRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%
\Symb{texCartesian}%
   {расслоение}%
   {bundle}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb{texCartesian}%
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%
\Symb{texBasis}%
   {активное преобразование}%
   {active transformation}%
\Symb{texAffine}%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb{texVectorSpace}%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb{texAffine}%
   {кривизна}%
   {GLn curvature_overline}%
\Symb{texVectorSpace}%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb{texRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texRepresentation}%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb{texVectorSpace}%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%
\Symb{texLie}%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%
\Symb{texBasis}%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb{texBasis}%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb{texVectorSpace}%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb{texLinearMap}%
   {($S$, $T$)\hyph бимодуль}%
   {R S bimodule}%
\Symb{texVectorSpace}%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb{texVectorSpace}%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb{texBasis}%
   {векторное пространство}%
   {V}%
\Symb{texReferenceFrame}%
   {векторное пространство векторных полей}%
   {vector space of vector fields}%

\SetIndexSpace%
\Symb{texPolymodule}%
   {геометрический объект в координатном представлении,		определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\Symb{texPolymodule}%
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%

\SetIndexSpace%
\Symb{texTidal}%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb{texRepresentation}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texTstarMorphism}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texBasis}%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb{texBiring}%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb{texAffine}%
   {символ Картана}%
   {Cartan symbol}%
\Symb{texAffine}%
   {связность}%
   {conection overline}%
\Symb{texAffine}%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb{texCartesian}%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%
\Symb{texLie}%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb{texLie}%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, skew field}%
\Symb{texReferenceFrame}%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%

\SetIndexSpace%
\Symb{texLie}%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb{texBundleRelation}%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

